Learning Correspondence for Deformable Objects

We investigate the problem of pixelwise correspondence for deformable objects, namely cloth and rope, by comparing both classical and learning-based methods. We choose cloth and rope because they are traditionally some of the most difficult deformable objects to analytically model with their large configuration space, and they are meaningful in the context of robotic tasks like cloth folding, rope knot-tying, T-shirt folding, curtain closing, etc. The correspondence problem is heavily motivated in robotics, with wide-ranging applications including semantic grasping, object tracking, and manipulation policies built on top of correspondences. We present an exhaustive survey of existing classical methods for doing correspondence via feature-matching, including SIFT, SURF, and ORB, and two recently published learning-based methods including TimeCycle and Dense Object Nets. We make three main contributions: (1) a framework for simulating and rendering synthetic images of deformable objects, with qualitative results demonstrating transfer between our simulated and real domains (2) a new learning-based correspondence method extending Dense Object Nets, and (3) a standardized comparison across state-of-the-art correspondence methods. Our proposed method provides a flexible, general formulation for learning temporally and spatially continuous correspondences for nonrigid (and rigid) objects. We report root mean squared error statistics for all methods and find that Dense Object Nets outperforms baseline classical methods for correspondence, and our proposed extension of Dense Object Nets performs similarly.

==> references/preamble_algo.tex <==
%!TEX root = main.tex
\lstdefinelanguage{mine} 
{morekeywords={while,True,if,break,=,return,function,for,until,in,input,output,assumptions,assumption,invariant,loop,variant,end,invariant,precondition,variables}, 
sensitive=false, 
morecomment=[l]{\#}, 
morecomment=[il]\%{.}, 
morecomment=[s]{/*}{*/}, 
morestring=[b]", 
} 

\lstset{% general command to set parameter(s) 
basicstyle=\small\rmfamily, % print whole listing small 
keywordstyle=\color{black}\bfseries, 
% underlined bold black keywords 
identifierstyle=, % nothing happens 
commentstyle=\color[rgb]{0.2,0.2,0.2},
stringstyle=\ttfamily, % typewriter type for strings 
showstringspaces=false,
mathescape=true,
fontadjust=true,
columns=fullflexible} % no special string spaces 
\lstset{frameround=fttt,frame=none}

\usepackage{calc}
\newlength\listingnumberwidth
\setlength\listingnumberwidth{\widthof{00}}
\lstset{
numbers=left,
xleftmargin=\listingnumberwidth,
numbersep=1em
}


\lstset{escapeinside={*@}{@*}}

\newcommand{\tuple}[2]{\langle#1,#2\rangle}

==> tex/EM-old.tex <==
%!TEX root = ../main.tex

\section{An Expectation-Maximization Approach to Multi-Model Registration}
\label{sec:xxx}



% \subsection{Sushrut's Algorithm}
% \snote{Probably need to remove this subsection.}
% First, we calculate all expectation for all the possible monomials of $x$ components.
% $$
% (S_x)_{i} = [x_{i,a} x_{i,b} x_{i,c}],
% $$
% where $(a, b, c) \in [D]^3$ and $(S_x)_i$ is each row of $S_x$ whose size is $D^3 \times N$.
% Then, we calculate the triple of power of the $y$ values.
% $$
% (S_y)_i = y_{i}^3,
% $$
% where $S_y$ has a size of $D^3 \times 1$ 

% \begin{align*}
%     E_{xx} &= E[(S_x)_i (S_x)_i^T] \\
%     E_{xy} &= E[(S_y)_i (S_x)_i]  
% \end{align*}

% We perform an
% $$
% E_w = E_{xx}^{\dagger} E_{xy}
% $$ and convert this into a $D \times D \times D$ symmetric matrix.

% Lastly, we use a subspace power method to perform tensor decomposition on $E_w$ to recover up to $D$ vectors with size $D \times 1$.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Expectation-Maximization Algorithm}
% \snote{Can we get rid of this section and send everything to the algorithm? We have basically done this already.} 
% The goal of the Classification Expectation-Maximization (CEM) 
% algorithm (described in \Cref{alg:EM}), is (given a good initialization),
% to recover the ground truth clustering.
% We do this of the model by maximizing the following likelihood function
% $$
% L(\theta | \va_1, ..., \va_n, \vb_1, ..., \vb_n)  = \sum_{i=1}^{N} \log \left ( \sum_{k=1}^H \pi_k \phi(\vb_i | \va_i) \right ),

The Expectation-Maximization (EM) algorithm iteratively estimates parameters in statistical models given noisy data, by alternating two kinds of steps. 
An E-step to compute expected hidden values (in our case these are the poses $(\MR_j,\vt_j)$ of the objects), and a M-step to update parameters based on those expected hidden values (in our case the parameters are the vectors $\vtheta_i$ associating each measurement to a specific object). 
We use a variant of the Expectation-Maximization (EM) algorithm (\Cref{alg:EM}) that we describe below.
% to recover the associations between measurements and objects (including background) as well as the motion of each object. 
% We describe the algorithm below. 



\myparagraph{Preliminaries and Notation}
% We provide the following notation and definitions that we will use in this and the following section. 
We say that a set of points $S$ is 
\emph{$\tau$-connected} if between any pair of points $\vxx, \vy \in S$ there is a sequence of points in $S$ such that each pair of consecutive points in the sequence are at most at distance $\tau$ from each other. 
For a set of points $C$, 
we define $d_{\text{cluster}}(C, \vp)$ to be the minimum distance between $C$ and the point $\vp$, i.e. $ d_{\text{cluster}}(C, \vp) := \min_{\vp' \in C} \norm{\vp' - \vp}$. {We will also sometimes use $\vp$ to denote $(\va, \vb) \in \mathbb R^3 \times \mathbb R^3$.}
Now we observe that finding the associations can be thought of as a \emph{clustering} problem, where we are trying to cluster together measurements corresponding to the same object. 
We will refer to our clusters with $H_j \subset S$, where $S$ is the initial set of points and $H_j$ indicates the point (or more precisely, the correspondences) associated with object $j$. 
Note that this interpretation is consistent with~\eqref{eq:measModel3}, and 
by definition $H_j := \{ (\va_i, \vb_i) \in S \mid \theta_{i,j} = 1 \}$.
 Accordingly, in \Cref{alg:EM}, rather than updating the indicator vectors $(\vtheta)$, 
 we update the clusters $H_j$ for all $j$.

\myparagraph{Initialization} 
Similar to theoretical analyses of the EM algorithm in prior work in the context of learning a mixture of linear regressions, we require a good initialization (see, for e.g. \cite{kwon20aistats-EM-MLR}). However, these analyses are very specific to the case where the measurements are Gaussian and their initialization does not apply to real-world settings. 
We instead define a notion of good initialization which we can achieve using preexisting algorithms 
% to get an initial clustering of the given point cloud, 
and show that \Cref{alg:EM} converges given such an initialization.

The algorithm takes as input, an initial clustering 
$\cH := \{H_j \subset S \mid j \in [k]\}$ of the point cloud 
$S = \{ (\va_i, \vb_i) \}_{i=1}^{n}$ 
satisfying certain conditions (which we observe in our experiments),
namely, (i) $\cH$ is a partition of $S$;
(ii) Every ground truth cluster contains at least one cluster from $\cH$ that is relatively large compared to the others; and
(iii) Every cluster in the initial clustering is not too small, and is $\tau$-connected.

 

% , for some $T \in \mathbb N$, there is a path $\vxx, \vp_1, \dots, \vp_T, \vy$ , such that $\max \{ \norm{\vxx - \vp_1}, \norm{\vp_T - \vy } \} \cup \{ \norm{\vp_i - \vp_{i+1}} \mid i\in[T-1] \} \leq \tau$. 
\input{tex/alg}

\myparagraph{EM Algorithm} Each iteration of \Cref{alg:EM} performs an E-step and M-step. 
The E-step estimates the posterior probability that the data point 
$(\va_i, \vb_i)$ belongs to the cluster $j$ after the $r$-th iteration according to the weighted likelihood \begin{equation}
W^{(r)}_{i,j;\tau} :=\frac{\pi_j^{(r)} \phi^{(r)}(\vb_i | \va_i)}{\sum_{j=1}^{k} \pi_j^{(r)} \phi^{(r)}(\vb_i | \va_i) } \cdot \mathbf{1}(d_{\text{cluster}}(H_j, (\va_i, \vb_i)) < \tau).
\label{eq:likelihood}
\end{equation}
The distance term $\mathbf{1}(d_{\text{cluster}}(H_j, (\va_i, \vb_i)) < \tau)$ aims to capture the fact that the ground truth is $\tau$-connected. Here $\phi_j(\vb_i|\va_i)$ denotes the the likelihood of $\vb_i - \MR_j \va_i - \vt_j$ with respect to the independent multivariate Gaussian density with mean $0$ and covariance $\sigma_j^2 I_3$, where $(\MR_j, \vt_j)$ is the rigid transformation and $\pi_j$ is the weight for cluster $j$.

Then, in M-step, the algorithm updates the $(r+1)$-th 
assignment of samples to the clusters ($\cH$) by assigning each sample to the cluster maximizing $W^{(r)}_{i,j;\tau}$. 
This particular variation of the M-step is called the ``Classification M-step", and this variation of the EM algorithm is referred to as the ``Classification Expectation-Maximization" algorithm (see, for e.g. \cite{FariaSoromenho10}). 

In the algorithm \ref{alg:EM}, we use Horn's method \cite{ Arun87pami, Horn87josa} to calculate the hypothesis for each new cluster and we delete small point clouds so that the SVD is full rank.

In the following section, we demonstrate theoretical justification for our empirical observations, that given a good initialization, \Cref{alg:EM} converges to the ground truth clusters. 



% the expectation of the complete-data log-likelihood conditional on the current parameter estimates and the observed data by calculating the new weights and performing weighted least square regression on the data.

% We use the classification EM algorithm which incorporates a classification step (C step) between E-step and M-step. 
% classified EM. Instead of assigning a normalized likelihood value of 

% update new hypothesis

% distance term

% \begin{align*}
% \pi_k^{(r+1)} &= \frac{\sum_{i=1}^N w_{i,j}^{(r)}}{N} \\
% R_k^{(r+1)} &= (X^T W_k X)^{-1} (X^T W_k Y) \\
% \sigma_k^{(r+1)} &= 
% \end{align*}
% \snote{Fix $R_k$ -- this is done using Horn's method (i.e. use centroid using rotation matrix) ALSO we use CEM -- the thing written here is EM. The algorithm is correct; also $\sigma_k$ is just the variance of $Ra + t - b$ restricted to $k$.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \new{What we need to show: 

% 1. If we don't throw a hypothesis it either becomes closer to 
% 2. 

% }


% The proof of this 





% We need to demonstrate two things.
% First, if a hypothesis is far from any element in $\cG$, 
% then this hypothesis is eliminated at some stage.
% Second, for every hypothesis in $\cG$, there is a hypothesis
% in $\cH$ that is $\eta$-close in $2$-norm.

% For each hypothesis $(G, g) \in \cG$ let $O_{(G, g)}$ denote
% the set of points corresponding to this ground truth-hypothesis. 
% Also, for each hypothesis $(H, h)$ 
% let $S_{(H, h); \eta'}$ denote the set of samples
% which satisfy $\norm{ Hx + h - y } \leq \eta'$.


% \paragraph{Hypothesis elimination}
% Since \Cref{ass:anticoncentration_cluster} holds, 
% we know that any $\gamma$-fraction $O_{\gamma}$ of $O_{(G, g)}$
% satisfies $\E_{(x, y) \sim O_\gamma}[ xx^T ] \succcurlyeq \tau I_d$. 
% This means that if $|S_{(H,h)} \cup O_{(G, g)}| \geq \gamma |O_{(G, g)}|$,
% then for all the points in the intersection, 
% $\norm{ Hx + h - y } \leq \eta'$ and $\norm{Gx + g - y} \leq \eta'$
% and so $\norm{(H-G)x + (h-g)}^2 \leq 4\eta'^2$. 
% Taking an expectation over points in $S_{(H,h)} \cup O_{(G, g)}$ implies
% $\E[\norm{(H-G)x + (h-g)}^2] \leq 4\eta'^2$


% However, this cannot happen since we assumed that $(H, h)$ is far
% from every $(G, g)$. 

% \new{Note that every inlier is very likely to be assigned to one of the elements of $\cG$.} 

% Suppose $(H, h)$ is far away, then by \new{ \Cref{ass:large_clusters} } it 
% has a small intersection with every ground truth cluster.
% i.e. only $(1-\eta) \cdot |\cG| \leq (1-\eta)/\gamma$ points are explained by $(H, h)$. 
% This means, in step 4 of \Cref{alg:EM} the hypothesis gets eliminated. 
% \snote{By choosing $\eta$ and $\gamma$ correctly we should be done.}


% To see that no hypothesis in $\cG$ is ever eliminated,
% observe that every hypothesis in $\cG$ initially is assigned 
% at least a $1/100$ fraction of the data points.
% We will show that 
% (1) at each step, there exists a hypothesis which matches the hypothesis
% in $\cG$ exactly, and,
% (2) at no point will the hypothesis be assigned less than 4 points. 



% By Assumption 1. We see that initially, the most likely hypothesis
% for each point is indeed its corresponding ground truth cluster. 
% To see (1), observe that among the initial hypotheses,
% we have for every hypothesis in $\cG$, a set of points for which
% this is an exact regressor. 


% note that every pair of hypotheses is at least $\alpha$ apart.
% }

==> tex/EM.tex <==
%!TEX root = ../main.tex

% \vspace{-7mm}
\section{An Expectation-Maximization Approach to Multi-Model Registration}
\label{sec:xxx}

% \subsection{Sushrut's Algorithm}
% \snote{Probably need to remove this subsection.}
% First, we calculate all expectation for all the possible monomials of $x$ components.
% $$
% (S_x)_{i} = [x_{i,a} x_{i,b} x_{i,c}],
% $$
% where $(a, b, c) \in [D]^3$ and $(S_x)_i$ is each row of $S_x$ whose size is $D^3 \times N$.
% Then, we calculate the triple of power of the $y$ values.
% $$
% (S_y)_i = y_{i}^3,
% $$
% where $S_y$ has a size of $D^3 \times 1$ 

% \begin{align*}
%     E_{xx} &= E[(S_x)_i (S_x)_i^T] \\
%     E_{xy} &= E[(S_y)_i (S_x)_i]  
% \end{align*}

% We perform an
% $$
% E_w = E_{xx}^{\dagger} E_{xy}
% $$ and convert this into a $D \times D \times D$ symmetric matrix.

% Lastly, we use a subspace power method to perform tensor decomposition on $E_w$ to recover up to $D$ vectors with size $D \times 1$.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Expectation-Maximization Algorithm}
% \snote{Can we get rid of this section and send everything to the algorithm? We have basically done this already.} 
% The goal of the Classification Expectation-Maximization (CEM) 
% algorithm (described in \Cref{alg:EM}), is (given a good initialization),
% to recover the ground truth clustering.
% We do this of the model by maximizing the following likelihood function
% $$
% L(\theta | \va_1, ..., \va_n, \vb_1, ..., \vb_n)  = \sum_{i=1}^{N} \log \left ( \sum_{k=1}^H \pi_k \phi(\vb_i | \va_i) \right ),

Here, we give a brief review of the algorithmic proposed in \cite{jin2024multimodel}. We start by recalling that the Expectation-Maximization (EM) algorithm~\cite{Moon96spm} iteratively estimates parameters in statistical models given noisy data, by alternating an Expectation (E) step and a Maximization (M) step. 
In robotics, EM has been a popular approach to attack estimation problems including discrete and continuous variables~\cite{Eckart18cvpr-HGMR, Rogers10IROS-EMslam,Indelman14ICRA-posegraph,Bowman17icra}.
In \cite{jin2024multimodel}, the authors propose to use a variation of the EM algorithm known as the ``Classification Expectation-Maximization'' algorithm (\eg~\cite{FariaSoromenho10}), see~\Cref{alg:EM}. 
% in the robotics literature, \eg \cite{Rogers10IROS-EMslam,Indelman14ICRA-posegraph}, the M step computes a guess for the discrete variables, while the E step computes an estimate for the continuous variables.
% % variables of interest (\eg $(\MR_j,\vt_j)$) given the associations.
% % \cite{Rogers10IROS-EMslam}
% In this paper, we consider a different variation of the EM algorithm, where both the E and the M 
% steps  
% An E-step to compute expected hidden variables (in our case these are the poses $(\MR_j,\vt_j)$ of the objects), and a M-step to update parameters based on those expected hidden values (in our case the parameters are the vectors $\vtheta_i$ associating each measurement to a specific object). 
% We use a variant of the EM algorithm (\Cref{alg:EM}) that we describe below.
% to recover the associations between measurements and objects (including background) as well as the motion of each object. 
% We describe the algorithm below. 
\input{tex/alg_e}

We summarize how the algorithm works here. With the observation that finding the associations $\vtheta_i$ can be equivalently thought of as a \emph{clustering} problem, the algorithm at its core tries to cluster together measurements corresponding to the same object. 
We will refer to the clusters as $H_j \subset S$, where $S$ is the given set of correspondences $\{ (\va_i, \vb_i)\}_{i=1}^n$ and $H_j$ indicates the correspondences (putatively) associated with object $j$. 
Note that this interpretation is consistent with~\eqref{eq:measModel3}, and 
by definition $H_j := \{ (\va_i, \vb_i) \in S \mid \theta_{i,j} = 1 \}$.
 Accordingly, in \Cref{alg:EM}, rather than updating the indicator vectors $\vtheta_i$, 
the clusters $H_j$ are updated for all objects $j$, at each iteration.

\myparagraph{Initialization}
The algorithm takes as input, an initial guess for the clusters 
$\cH := \{H_j \subset S \mid j \in [K]\}$ of the correspondences
$S$, %= \{ (\va_i, \vb_i) \}_{i=1}^{n} 
where for each object $j \in [K]$, $H_j$ is the set of correspondences associated to $j$. In the next section, we provide conditions on the initialization under which the EM algorithm converges to the ground truth.
% and in Section~\ref{sec:experiments} 
 % we show that is relatively easy to satisfy these conditions.
% while in the experiments we verify
% that such conditions are indeed mild. 
% \red{$\frac{\pi_j^{(r)} \phi^{(r)}(\vb_i | \va_i)}{\sum_{j=1}^{k} \pi_j^{(r)} \phi^{(r)}(\vb_i | \va_i) } \mathbf{1}(d_{\text{cluster}}(H_j, (\va_i, \vb_i)) < \tau)$}

% , for some $T \in \mathbb N$, there is a path $\vxx, \vp_1, \dots, \vp_T, \vy$ , such that $\max \{ \norm{\vxx - \vp_1}, \norm{\vp_T - \vy } \} \cup \{ \norm{\vp_i - \vp_{i+1}} \mid i\in[T-1] \} \leq \tau$. 
% \input{tex/alg}

\myparagraph{EM Algorithm} Each iteration of \Cref{alg:EM} performs an E-step and M-step. 
At each iteration $r$, the algorithm first computes a transform $(\MR_j^{(r)}, \vt_j^{(r)})$ for each cluster (line~\ref{line:procrustes}); this is done using Horn's method \cite{Horn87josa} given the measurements in that cluster.
%to calculate the hypothesis for each new cluster and we delete small point clouds so that the SVD is full rank.
The algorithm also computes a weight $\pi_j^{(r)}$ (quantifying the relative size of  cluster $j$) and an intra-cluster variance $\hat\sigma_j^{(r)}$ for each cluster (lines~\ref{line:weight}-\ref{line:variance}). 
Then, the E-step estimates the posterior probability that the data point 
$(\va_i, \vb_i)$ belongs to the cluster $j$ according to the weighted likelihood:

 \begin{equation}
W^{(r)}_{i,j;\tau} :=\frac{\pi_j^{(r)} \phi^{(r)}(\vb_i | \va_i)}{\sum_{j=1}^{k} \pi_j^{(r)} \phi^{(r)}(\vb_i | \va_i) } \cdot \mathbf{1}(d_{\text{cluster}}(H_j, (\va_i, \vb_i)) < \tau).
\label{eq:likelihood}
\end{equation}
Here $\phi_j^{(r)}(\vb_i|\va_i)$ denotes the likelihood of $\vb_i - \MR_j^{(r)} \va_i - \vt_j^{(r)}$ with respect to the  multivariate Gaussian density with mean $\zero$ and covariance $\hat\sigma_j^2 \eye_3$. 
%, where $(\MR_j, \vt_j)$ is the rigid transformation associated to cluster $j$.
The first term of the likelihood essentially quantifies how well the transformation $(\MR_j^{(r)},\vt_j^{(r)})$ agrees with the correspondence $(\va_i,\vb_i)$; the weighted likelihood also accounts for the cluster size (\ie the weight $\pi_j$). 
The second term $\mathbf{1}(d_{\text{cluster}}(H_j, (\va_i, \vb_i)) < \tau)$ assigns zero likelihood to points that are far away (farther than a distance $\tau$) from cluster $j$,  
where  
% In particular, %$d_{\text{cluster}}(C, \vp)$ to be the minimum distance between $C$ and the point $\vp$, i.e. 
$ d_{\text{cluster}}(H_j, (\va_i, \vb_i)) := \min_{\va' \in H_j} \norm{\va' - \va_i}$. 
%{We will also sometimes use $\vp$ to denote $(\va, \vb) \in \mathbb R^3 \times \mathbb R^3$.
This term avoids to cluster together objects that might have the same motion, but are far away from each other. 
%aims to capture the fact that the ground truth is $\tau$-connected. 
% For a set of points $C$, 
% we define $d_{\text{cluster}}(C, \vp)$ to be the minimum distance between $C$ and the point $\vp$, i.e. $ d_{\text{cluster}}(C, \vp) := \min_{\vp' \in C} \norm{\vp' - \vp}$. {We will also sometimes use $\vp$ to denote $(\va, \vb) \in \mathbb R^3 \times \mathbb R^3$.

The M-step %, the algorithm updates the $(r+1)$-th 
updates the assignment of samples to the clusters by assigning each $(\va_i,\vb_i)$ to the cluster $H_j$ maximizing $W^{(r)}_{i,j;\tau}$. 
This particular variation of the M-step is called the ``Classification M-step'', see, \eg~\cite{FariaSoromenho10}. Before executing the M-step, the algorithm removes overly small clusters (line~\ref{line:remove}). 

% We remark that \Cref{alg:EM} is almost parameter free, and only requires setting the distance $\tau$ beyond which we consider two objects to be distinct, the minimum ``size'' $m_{\min}$ of what we would consider an object, and the number of iterations $T$. In particular, the weighted likelihood only depends on $\tau$ and does not require setting a noise bound, \eg as done in RANSAC.
% We also remark that the number of clusters $K$ is estimated during the iterations, and ideally will converge to the true number of objects $M$, see eq.~\eqref{eq:measModel3}.

% In the following section, we derive conditions under which 
% % the provide theoretical justification for our empirical observations, that given a good initialization, 
% \Cref{alg:EM} converges to the ground truth clusters. 


% the expectation of the complete-data log-likelihood conditional on the current parameter estimates and the observed data by calculating the new weights and performing weighted least square regression on the data.

% We use the classification EM algorithm which incorporates a classification step (C step) between E-step and M-step. 
% classified EM. Instead of assigning a normalized likelihood value of 

% update new hypothesis

% distance term

% \begin{align*}
% \pi_k^{(r+1)} &= \frac{\sum_{i=1}^N w_{i,j}^{(r)}}{N} \\
% R_k^{(r+1)} &= (X^T W_k X)^{-1} (X^T W_k Y) \\
% \sigma_k^{(r+1)} &= 
% \end{align*}
% \snote{Fix $R_k$ -- this is done using Horn's method (i.e. use centroid using rotation matrix) ALSO we use CEM -- the thing written here is EM. The algorithm is correct; also $\sigma_k$ is just the variance of $Ra + t - b$ restricted to $k$.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \new{What we need to show: 

% 1. If we don't throw a hypothesis it either becomes closer to 
% 2. 

% }


% The proof of this 





% We need to demonstrate two things.
% First, if a hypothesis is far from any element in $\cG$, 
% then this hypothesis is eliminated at some stage.
% Second, for every hypothesis in $\cG$, there is a hypothesis
% in $\cH$ that is $\eta$-close in $2$-norm.

% For each hypothesis $(G, g) \in \cG$ let $O_{(G, g)}$ denote
% the set of points corresponding to this ground truth-hypothesis. 
% Also, for each hypothesis $(H, h)$ 
% let $S_{(H, h); \eta'}$ denote the set of samples
% which satisfy $\norm{ Hx + h - y } \leq \eta'$.


% \paragraph{Hypothesis elimination}
% Since \Cref{ass:anticoncentration_cluster} holds, 
% we know that any $\gamma$-fraction $O_{\gamma}$ of $O_{(G, g)}$
% satisfies $\E_{(x, y) \sim O_\gamma}[ xx^T ] \succcurlyeq \tau I_d$. 
% This means that if $|S_{(H,h)} \cup O_{(G, g)}| \geq \gamma |O_{(G, g)}|$,
% then for all the points in the intersection, 
% $\norm{ Hx + h - y } \leq \eta'$ and $\norm{Gx + g - y} \leq \eta'$
% and so $\norm{(H-G)x + (h-g)}^2 \leq 4\eta'^2$. 
% Taking an expectation over points in $S_{(H,h)} \cup O_{(G, g)}$ implies
% $\E[\norm{(H-G)x + (h-g)}^2] \leq 4\eta'^2$


% However, this cannot happen since we assumed that $(H, h)$ is far
% from every $(G, g)$. 

% \new{Note that every inlier is very likely to be assigned to one of the elements of $\cG$.} 

% Suppose $(H, h)$ is far away, then by \new{ \Cref{ass:large_clusters} } it 
% has a small intersection with every ground truth cluster.
% i.e. only $(1-\eta) \cdot |\cG| \leq (1-\eta)/\gamma$ points are explained by $(H, h)$. 
% This means, in step 4 of \Cref{alg:EM} the hypothesis gets eliminated. 
% \snote{By choosing $\eta$ and $\gamma$ correctly we should be done.}


% To see that no hypothesis in $\cG$ is ever eliminated,
% observe that every hypothesis in $\cG$ initially is assigned 
% at least a $1/100$ fraction of the data points.
% We will show that 
% (1) at each step, there exists a hypothesis which matches the hypothesis
% in $\cG$ exactly, and,
% (2) at no point will the hypothesis be assigned less than 4 points. 



% By Assumption 1. We see that initially, the most likely hypothesis
% for each point is indeed its corresponding ground truth cluster. 
% To see (1), observe that among the initial hypotheses,
% we have for every hypothesis in $\cG$, a set of points for which
% this is an exact regressor. 


% note that every pair of hypotheses is at least $\alpha$ apart.
% }

==> tex/abstract.tex <==
%!TEX root = ../main.tex

\begin{abstract}
We perform detailed theoretical analysis of an expectation-maximization-based algorithm recently proposed in \cite{jin2024multimodel} for solving a variation of the 3D registration problem, named \emph{multi-model 3D registration}. Despite having shown superior empirical results, \cite{jin2024multimodel} did not theoretically justify the conditions under which the EM approach converges to the ground truth. In this project, we aim to close this gap by establishing such conditions. In particular, the analysis revolves around the usage of probabilistic tail bounds that are developed and applied in various instances throughout the course. The problem studied in this project stands as another example, different from those seen in the course, in which tail bounds help advance our algorithmic understanding in a probabilistic way. We provide self-contained background materials on 3D Registration. %In the \nameProblemLong problem, we are given two point clouds picturing a set of objects at different poses (and possibly including points belonging to the background) and we want to simultaneously reconstruct how all objects moved between the two point clouds.
%the motion of all the objects between the point clouds.
 %This setup generalizes standard 3D registration where one wants to reconstruct a single pose, \eg the motion of the sensor picturing a static scene. Moreover, it provides a mathematically grounded formulation for relevant robotics applications, \eg where a depth sensor onboard a robot perceives a dynamic scene and has the goal of estimating its own motion (from the static portion of the scene) while simultaneously recovering the motion of all dynamic objects. 
 % \eg two RGB-D scans taken at consecutive times, that picture a collection of rigid objects, moving with respect to each. Then the goal is to simultaneously compute the relative pose for each object in the cloud. This generalizes the typical registration setup where one attempts to recover a single pose. 
%We assume a correspondence-based setup where we have putative matches between the two point clouds and consider the practical case where these correspondences are plagued with outliers.
%We use probabilistic bounds learned from the class to establish theoretical conditions under which the EM approach converges to the ground truth with high probability.
% We then propose a simple approach based on Expectation-Maximization (EM) and 
% % but ---contrary to related work--- we 
% establish theoretical conditions under which the EM approach converges to 
% the ground truth. We evaluate the approach in simulated and real datasets ranging from table-top 
% scenes to  self-driving scenarios and demonstrate its effectiveness 
% in conjunction with state-of-the-art %learning-based 
% scene flow methods for dense correspondences.
% when combined with state-of-the-art %learning-based 
% scene flow methods %(\ie RAFT) 
% to establish dense correspondences.  
\end{abstract}

==> tex/alg.tex <==
%!TEX root = ../main.tex

\begin{algorithm}[t]
\caption{Expectation-Maximization (EM)}
\label{alg:EM}
\SetAlgoLined
\small
\begin{algorithmic}[1]
\STATE \textbf{Input:}
 Point clouds $S := \{(\va_i,\vb_i)\}_{i=1}^n$,
Initial clusters $\cH := \{H_j \subset S \mid j \in [K] \}$, 
Threshold $\tau$, 
Number of iterations $T$,
Minimum cluster size $m_{\min}$
% \vspace{1mm}
% \STATE 
% Define the following: \\
% Initial assignment: For $\vp \in S$, $\alpha(\vp) := i$ where $\vp \in H_i$. \\
% Initial weighted likelihood: $W_{i,j; \infty}^{(0)} := 1$ \\
\smallskip

\FOR{$r \in [T]$}

\STATE {\color{gray} \% Compute a pose, weight, and variance for each cluster}
\FOR{$j \in [K]$}
% \STATE Remove those hypotheses with very few samples assigned to them, and update the rest via Horn's method.
% \vspace{3mm}

\STATE $(\MR_j^{(r)}, \vt_j^{(r)}) := \text{Horn}(H_j)$. \label{line:procrustes} \\
\STATE  $\pi_j^{(r)} := |H_j|/n$. \label{line:weight} \\
% |H_i|/m
% \text{This is initially the size of cluster $k$ over total sample size.}\\
% \text{$E_j$ denotes the following set of errors} 
\STATE  $E_{j} := \{ \vb - \MR_j^{(r)} \va - \vt_j^{(r)} \mid (\va, \vb) \in H_j \}$\\
 \STATE $\sigma_j^{(r)} := \sqrt{ \frac{1}{3} \trace{ \text{cov}(E_j) }}$ \label{line:variance} 
%\sqrt{ (1/3)\sum_{q=1}^3 \textit{Var}(E_j \cdot e_q) }$
\ENDFOR
\smallskip
\textbf{E-step:}\\
\smallskip
% \vspace{3mm}
\FOR{$j \in [K]$ and $i \in [n]$}  
% \STATE Estimate the weighted likelihood:
\STATE    $ W_{i,j; \tau}^{(r)}$ := eq.~\eqref{eq:likelihood}
    %\text{Likelihood}(\MR_j^{(r)},\vt_j^{(r)},\sigma_j^{(r)},\va_i,\vb_i,\tau)$
% \STATE where $\pi_j$ is the weight for hypothesis; $\phi_j(\vb_i|\va_i)$ denotes the independent multivariate Gaussian density of $\vb_i$ for mixture $j$ with $h_j(\va_i)$ as mean and $\sigma_k^2 I_3$ as covariance. 
\ENDFOR
% of $\vb_j$ being generated from $\va_j$ using the hypothesis $h_i$, 
% when the noise is Gaussian with standard deviation $\sigma$. 
% Here $\phi_\sigma(\cdot)$ is the PDF of a Gaussian distribution with variance $\sigma^2$.\\
\smallskip
\STATE {\color{gray} \% Remove small clusters $H_j$ from $\cH$}
\FOR{$j \in [K]$}
\IF{$|H_j| < m_{\min}$} 
\STATE remove cluster $j$ from $\calH, \pi_j^{(r)}, \sigma_j^{(r)}, W_{i,j; \tau}^{(r)}$
\STATE $K := K - 1$ 
\ENDIF
\ENDFOR
\smallskip
\textbf{M-Step:}\\
\smallskip
\STATE {\color{gray} \% Update clusters} %  $\vtheta_i^{(r)}$
\FOR{ $i \in [n]$}
\STATE if $j^\star = \argmax_{j \in [k]} W^{(r)}_{i, j;\tau}$, add $(\va_i, \vb_i)$ to cluster $H_{j^\star}$
%$\alpha^{(r)}((\va_i, \vb_i)) := \argmax_{j \in [k]} W^{(r)}_{i, j;\tau}$.
\ENDFOR
% \STATE Update $\cH$ to be $\{ {\alpha^{(r)}}^{-1}(j) \mid i \in [k] \}$.

\ENDFOR
\RETURN $H_j, \MR_j^{(r)}, \vt_j^{(r)}, \text{ for} j=1,\ldots,K$.
\end{algorithmic}
\vspace{-4mm}
\end{algorithm}

==> tex/alg_e.tex <==
%!TEX root = ../main.tex

\begin{algorithm}
\caption{Expectation-Maximization (EM)}
\label{alg:EM}
\SetAlgoLined
\small
\KwIn{
 Point clouds $S := \{(\va_i,\vb_i)\}_{i=1}^n$,
Initial clusters $\cH := \{H_j \subset S \mid j \in [K] \}$, 
Distance threshold $\tau$, 
Number of iterations $T$,
Minimum cluster size $m_{\min}$}
\KwOut{$H_j, \MR_j^{(r)}, \vt_j^{(r)}, \forall j \in [K]$}
% \vspace{1mm}
% \STATE 
% Define the following: \\
% Initial assignment: For $\vp \in S$, $\alpha(\vp) := i$ where $\vp \in H_i$. \\
% Initial weighted likelihood: $W_{i,j; \infty}^{(0)} := 1$ \\
\smallskip

\For{$r \in [T]$}{

{\color{gray} \% Compute a pose, weight, and variance for each cluster}
\For{$j \in [K]$}{
% \STATE Remove those hypotheses with very few samples assigned to them, and update the rest via Horn's method.
% \vspace{3mm}

$(\MR_j^{(r)}, \vt_j^{(r)}) := \text{Horn}(H_j)$. \label{line:procrustes}
$\pi_j^{(r)} := |H_j|/n$. \label{line:weight} \\
% |H_i|/m
% \text{This is initially the size of cluster $k$ over total sample size.}\\
% \text{$E_j$ denotes the following set of errors} 
$E_{j} := \{ \vb - \MR_j^{(r)} \va - \vt_j^{(r)} \mid (\va, \vb) \in H_j \}$\\
$\hat\sigma_j^{(r)} := \sqrt{ \frac{1}{3} \trace{ \text{cov}(E_j) }}$ \label{line:variance} 
%\sqrt{ (1/3)\sum_{q=1}^3 \textit{Var}(E_j \cdot e_q) }$
}
\smallskip
\textbf{E-step:} {\color{gray} \% Compute weighted likelihood:} \\
\smallskip
% \vspace{3mm}
\For{$j \in [K]$ and $i \in [n]$}{
% \STATE Estimate the weighted likelihood:
$ W_{i,j; \tau}^{(r)}$ := eq.~\eqref{eq:likelihood}
    %\text{Likelihood}(\MR_j^{(r)},\vt_j^{(r)},\sigma_j^{(r)},\va_i,\vb_i,\tau)$
% \STATE where $\pi_j$ is the weight for hypothesis; $\phi_j(\vb_i|\va_i)$ denotes the independent multivariate Gaussian density of $\vb_i$ for mixture $j$ with $h_j(\va_i)$ as mean and $\sigma_k^2 I_3$ as covariance. 
}
% of $\vb_j$ being generated from $\va_j$ using the hypothesis $h_i$, 
% when the noise is Gaussian with standard deviation $\sigma$. 
% Here $\phi_\sigma(\cdot)$ is the PDF of a Gaussian distribution with variance $\sigma^2$.\\
\smallskip
{\color{gray} \% Remove small clusters $H_j$ from $\cH$}

\For{$j \in [K]$ \label{line:remove}}{
\If{$|H_j| < m_{\min}$} {
remove cluster $j$ from $\calH, \pi_j^{(r)}, \hat\sigma_j^{(r)}, W_{i,j; \tau}^{(r)}$
$K := K - 1$ 
}
}
\smallskip
\textbf{M-Step:} {\color{gray} \% Regenerate clusters according to likelihoods} \\
\smallskip
%  $\vtheta_i^{(r)}$

\For{$i \in [n]$}{
\If{$j^\star = \argmax_{j \in [k]} W^{(r)}_{i, j;\tau}$}{
add $(\va_i, \vb_i)$ to cluster $H_{j^\star}$
%$\alpha^{(r)}((\va_i, \vb_i)) := \argmax_{j \in [k]} W^{(r)}_{i, j;\tau}$.
}
}
% \STATE Update $\cH$ to be $\{ {\alpha^{(r)}}^{-1}(j) \mid i \in [k] \}$.

}
% \KwRet{$H_j, \MR_j^{(r)}, \vt_j^{(r)}, \forall j \in [K]$}.
\end{algorithm}


==> tex/conclusion.tex <==
%!TEX root = ../main.tex

\section{Conclusion}
\label{sec:conclusion}
We reviewed and investigated an expectation-maximization-based algorithm recently proposed in \cite{jin2024multimodel} for solving a variation of the 3D registration problem, named \emph{multi-model 3D registration}, that simultaneously recovers the motion of multiple objects in point clouds. Building on the algorithm proposed therein, we established and proved theoretical conditions under which the EM scheme recovers the ground truth by employing the tail bounds developed in the course. These conditions characterize high-probability algorithmic convergence guarantees for this safety-critical robotics task. As another highlight, instead of omitting the asymptotic constants as having been done in the class, we kept them and avoided using big O notation as the robotics applications would require accurate constants to design for practical application.

% when combined with state-of-the-art scene flow methods to establish dense correspondences.
% While our method shows strong performance on a range of object classes, there is substantial room for improvement. One avenue for future work is to better design the likelihood function in the algorithm. Currently, we impose a hard threshold $\tau$ on the distance, we would like to find a better way to constrain distances between clusters. Robustness can also be improved both theoretically and algorithmically. We would like to replace the normal Horn's method with a more robust but still efficient point cloud registration method.

==> tex/experiments-long.tex <==
%!TEX root = ../main.tex

\begin{table}[]
\caption{Results for synthetic PASCAL3D+ dataset with and without Gaussian additive noise. Experiment 1: Noiseless. Experiment 2: with additive Gaussian noise. Experiment 3: with additive Gaussian noise and same-hypothesis objects}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
                                                                          & \multirow{2}{*}{Metric} & \multicolumn{4}{l}{Method}    \\
\cline{3-6}
                                                                          &                         & Ours & Ours (Vanilla) & T-Linkage & SRANSAC \\
                                                                          \hline
                                                                          \hline
\multirow{4}{*}{1}                                                        & Per-point Error    &   0.0525   &   0.0525        &    0.637 & 2.29     \\
                                                                          & Rotation error     &   0.0  &      0.0     &     1.2e-6  & 48.7     \\
                                                                          & Translation error  &   2.54e-14   &   2.53e-14        &    3.52e-14 & 6.44       \\
                                                                          & IoU                     &  0.941    &      0.940     & 0.847  &   0.490      \\
                                                                          \hline
\multirow{4}{*}{2}                                                        & Per-point Erro     &  0.241    &    0.241       &    0.67 & 2.22        \\
                                                                          & Rotation error     &   0.180   &     0.181      &    0.651 &  52.7       \\
                                                                          & Translation error  &   0.0227   &     0.0229      &     0.0876 & 6.28       \\
                                                                          & IoU                     &   0.937   &     0.935      &     0.836   & 0.489 \\ 
\hline
\multirow{4}{*}{3}                                                        & Per-point Error       &  0.196    &    0.186       &    0.631 & 2.73       \\
                                                                          & Rotation error     &   0.150   &     0.149      &  0.610 & 44.50     \\
                                                                          & Translation error  &   0.0217   &     0.0209      &  0.142 &  6.97   \\
                                                                          & IoU                     &   0.898   &     0.838      &      0.792 &  0.439 \\                                                               
\end{tabular}
}
\label{table:pascal3d}
\end{table}

\section{Experiments}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/icra24-results.pdf}
    \caption{Results of 3 different metrics on two real datasets: FlyingThings3D and KITTI} 
    \label{fig:boxplots-main}
\end{figure*}
\label{sec:experiments}
% To evaluate the performance of the proposed method, 
We conduct a wide range of experiments on both synthetic and real-world datasets. The synthetic datasets are  PASCAL3D+~\cite{Xiang14-Pascal3DPlus} and FlyingThings3D~\cite{Mayer16CVPR-FT3D} and the real-world dataset is from 
%an autonomous driving benchmark dataset 
KITTI~\cite{Geiger13IJRR-KITTI}. 
We test the proposed approach against Sequential RANSAC~\cite{Torr98royalp-seqransac} and T-Linkage~\cite{Magri14CVPR-tlinkage}, and show it
% We also illustrate the comparison with algorithms from both optimization-based and clustering-based multi-model fitting methods, which are Sequential RANSAC~\cite{Torr98royalp-seqransac} and T-Linkage~\cite{Magri14CVPR-tlinkage} respectively. For some of the methods, a good initial clustering is crucial to maximize the performance. We thus consider the same method with different initial clustering as different baselines.
dominates \red{these baselines} on the multi-model 3D registration problem, and its performance is further improved by using \red{SegmentAnything (SAM)} \cite{Kirillov23arxiv-SAM} as initialization.

\subsection{Datasets}
\myParagraph{PASCAL3D+}
PASCAL3D+ \cite{Xiang14-Pascal3DPlus} is a widely used synthetic computer vision dataset designed for 3D object understanding and pose estimation. We choose 7 standalone objects from the dataset and use the vertices data from their CAD models as object point clouds. To generate point cloud pairs $(\va, \vb)$, we randomly sample transformation matrices from $SE(3)$ and apply them to the selected point clouds. We thus have correspondences since $\vb$ is transformed from $\va$. We perform an Euclidean clustering step to obtain the initial clusters and then apply our proposed algorithm. We compare the predicted poses with the ground-truth $SE(3)$ poses and the predicted clusters with the ground-truth masks. We also test the ability to perform against noises by preparing synthetic datasets when Gaussian additive noise presents and to cluster two objects with the same hypothesis. Our algorithm with and without the distance term is tested.

\myParagraph{FlyingThings3D}
FlyingThings3D \cite{Mayer16CVPR-FT3D} dataset has randomly moving objects from ShapeNet ~\cite{Wu15cvpr-shapenets}. The dataset provides RGB images, masks, depth maps, and disparity maps. We constructed the point clouds with ground-truth scene flows by popping up 3D points
from disparity maps. 

In our method, to construct correspondences, we make use of the state-of-the-art scene flow model CamliRAFT \cite{Liu22CVPR-camliflow} on RGB images and randomly sampled point cloud $\va$ to get predicted scene flow $f$ and add predicted scene flow on the point cloud to get the next frame's point cloud $(\vb=\va + f)$. We then use SegmentAnything (SAM) \cite{Kirillov23arxiv-SAM} to get the masks as the initial clustering for our method. It is worth noting that while SAM is able to produce high-quality masks on images, the masks are always too fine-grained (for example, letters on a cereal box would be segmented as another cluster). Since we are interested in object-level masks, we use the fine-grained SAM masks as initialization and use our method to merge them in order to obtain object-level masks. The masks (clusters) provided in FlyingThings3D are also object-level masks, which are used as ground truth when compared with our method's output. We obtain ground-truth poses for each object by running SVD on each object's point cloud and its counterpart displaced by the ground-truth scene flow.

\myParagraph{KITTI}
The KITTI \cite{Geiger13IJRR-KITTI} scene flow dataset consists of 200 scenes split into training, validation, and testing datasets with RGB images and LIDAR point clouds. We only use the validation set because no ground-truth optical flow is provided in the testing set for us to evaluate. 

To run our proposed method, we follow the same steps done for the FlyingThings3D dataset to construct correspondences and obtain initial clustering. While KITTI does provide masks, the masks are semantic. For example, when multiple cars are in the scene, the cars will be separated from the background, but they will be clustered into one cluster representing all cars. Thus, to obtain the ground-truth masks, we perform Euclidean clustering only on the point clouds with the car label in the semantic map and merge everything else as background, resulting in a masked point cloud with a cluster for each car and another cluster for the background. Then, we calculate the pose for each cluster as the ground-truth pose for each segmentation mask, in the same manner using SVD as done for FlyingThings3D.

\subsection{Baselines}
In our experiments, we show the comparison of our method with two baselines: T-Linkage~\cite{Magri14CVPR-tlinkage} and Sequential RANSAC (SRANSAC)~\cite{Torr98royalp-seqransac}. T-Linkage represents the clustering-based multi-model fitting algorithm and SRANSAC represents the optimization-based method. We also include a Naive baseline by simply applying Horn's method on each initial cluster for comparison.

\myParagraph{T-Linkage} T-Linkage is the continuous and relaxed version of j-Linkage~\cite{Roberto08ECCV-jlinkage}. T-Linkage uses Tanimoto distance instead of Jaccard distance in j-Linkage to better represent the similarity between clusters. For each step, T-Linkage merges the most similar clusters until no two clusters' preference functions are orthogonal. For each point $i$, its preference function with cluster $j$ can be calculated with 
\begin{equation}
\phi(i, j)) = \begin{cases}
    \e^{- \|h_j a_i - b_i\|/\tau_t} & d \leq 5 \tau \\
    0 & d > 5 \tau \\
\end{cases}.
\end{equation}
The time constant $\tau_t$ represents the exponential decay rate in the preference function. 

\myParagraph{Sequential RANSAC} Sequential RANSAC builds upon RANSAC that can robustly fit a single hypothesis with a large number of outliers. Each time we apply RANSAC on the point cloud, we obtain a hypothesis and the points associated with it. By removing these points from the point cloud and performing RANSAC repeatedly until the point cloud is empty, SRANSAC is able to recover multiple hypotheses.

In KITTI and FlyingThing3D, to further ablate the effect of initial clustering, we run T-Linkage \cite{Magri14CVPR-tlinkage} and our method initialized with both SAM masks and Euclidean clustering.

% \bit
% \item Simulation experiments?
% \item Real tests?
% \eit

\subsection{Metrics}
To evaluate the performance of our algorithm compared with other baselines, we use three metrics that evaluate different aspects of the results.
\begin{itemize}
    \item \textbf{Point Error ($\downarrow$): }Evaluates the dense displacement between the point cloud after ground-truth transformation and after predicted transformation. The point error is defined as the average L2 distance (in meters) between each object in the point cloud masked over ground-truth masks.
    \item \textbf{Pose Error ($\downarrow$): }Evaluates the distance between the predicted poses and ground-truth poses. For each predicted mask, we find all the corresponding ground-truth masks that intersect with the predicted mask. For each object's predicted pose, we compare the translational and rotational errors as follows:  \textit{Translation Error}: The L2 distance between the inferred pose translation ($\mathbf{t}^{pred}$) and the ground-truth pose translation ($\mathbf{t}^{GT}$). \textit{Rotation Error}: The geodesic $SO(3)$ distance \cite{Pan23CORL-tax} between the predicted pose rotation ($\mathbf{R}^{pred}$) and the ground-truth rotation ($\mathbf{R}^{GT}$). The final pose error of each predicted mask is the weighted average of all pose errors and the weights are the ratios of intersections in the predicted mask.
    \item \textbf{Mask Quality ($\uparrow$)}: Evaluates the quality of the predicted masks by assigning a ground-truth mask to each mask with the largest intersection and calculating the average Intersection over Union (IOU) over each pair of masks.
\end{itemize}


\subsection{Results}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \centering
% \begin{tabular}{l|l|c|c|c|c|c}
% \hline
% \multirow{2}{*}{Dataset}  &     \multirow{2}{*}{Method}             & Error per point & Pose rotation error & Pose translation error & Mask IoU & Overcounted Masks \\
%                         &                 & (meter) & (degree) & (meter) & (\%) & (\#) \\
% \hline
% \hline
% \multirow{3}{*}{PASCAL3D+} & Seq. RANSAC      &                 &                     &                        &  &    \\
%                            & T-Linkage        &                 &                     &            &            &     \\
%                            & Ours             &                 &                     &           &             &     \\
% \hline
% \multirow{5}{*}{FlyingThings3D}             & Seq. RANSAC      &                 &                     &                   &     &     \\
%                            & T-Linkage        &                 &                     &         &               &     \\
%                            & T-Linkage w/ SAM &                 &                     &          &              &     \\
%                            & EM               &                 &                     &           &             &     \\
%                            & Ours             &                 &                     &           &             &     \\

% \hline
% \multirow{5}{*}{KITTI}                       & Seq. RANSAC      &                 &                     &                  &      &   -  \\
%                            & T-Linkage        &                 &                     &          &              &    - \\
%                            & T-Linkage w/ SAM &                 &                     &            &            &   -  \\
%                            & EM               &                 &                     &            &            &  -   \\
%                            & Ours             &                 &                     &              &          &  -  \\
% \hline
% \end{tabular}
% \end{table*}

\myParagraph{PASCAL3D+} We compare our method with T-Linkage \cite{Magri14CVPR-tlinkage} and Sequential RANSAC \cite{Torr98royalp-seqransac} for both cases with and without Gaussian additive noise. Our method and T-Linkage use Euclidean clustering with 100 initial clusters as initialization while Sequential RANSAC has no initialization. In Table \ref{table:pascal3d}, our method outperformed other methods for most metrics in both cases. Especially, when the additive noise exists, our method is still able to recover the hypothesis with low error and can correctly cluster point clouds almost perfectly. In Experiment 3, although pose and point errors are almost identical for both our methods, the one with distance constraint predicts better masks since it is able to separate two objects even when they share the same hypothesis.

\myParagraph{FlyingThings3D}
We show the comparison between our method and other baselines on FlyingThings3D in the left portion of Fig. \ref{fig:boxplots-main}. As shown in the boxplots, our method outperforms other baselines. In particular, our method recovers the object masks consistently and works well with different kinds of initialization methods. SRANSAC, although produces poses with low errors, suffers from generating accurate masks. In our observation, SRANSAC can mostly recover up to 2 moving objects. T-Linkage clusters the point cloud better using Euclidean clustering which is a weaker initialization method than SAM. T-Linkage cannot merge a large size of initial clustering well as it only merges two clusters in each step and requires the calculation of similarities between every two clusters. Therefore, since SAM generates a more fine-grained initialization, Euclidean clustering becomes a better choice than SAM. SAM could be improved by tuning the parameters that generate a smaller number of masks that still cover the whole RGB image.
% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/gray.eps} \vspace{-3mm}
%     \caption{
%         Boxplots for Flyingthings3d} \vspace{-5mm} 
%         \label{fig:coverfigure}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\myParagraph{KITTI}
In the right portion of Fig. \ref{fig:boxplots-main}, we compare our method and other baselines on the KITTI dataset. Similar to its performance on FlyingThings3D, our method outperforms other baselines, especially in mask IOU and point error, and matches the results of SRANSAC which gives the best pose error. However, SRANSAC fails to consistently recover accurate masks. Interestingly, SRANSAC \cite{Torr98royalp-seqransac} does much better on the KITTI dataset than on the FlyingThings3D dataset. Compared to FlyingThings3D's results, the results on KITTI had fewer outliers and the effect of initial clustering is minimal. Note that CamLiRAFT produces higher quality scene flows for the KITTI dataset as compared to the FlyingThings3D dataset as its KITTI checkpoint is fine-tuned on the FlyingThings checkpoint. This explains why the mask result for KITTI is overall better than the one for FlyingThings despite KITTI is a real-world dataset.
% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/gray.eps} \vspace{-3mm}
%     \caption{
%         Boxplots for KITTI} \vspace{-5mm} 
%         \label{fig:coverfigure}
% \end{figure}

==> tex/experiments.tex <==
%!TEX root = ../main.tex

\section{Experiments}

\label{sec:experiments}
% To evaluate the performance of the proposed method, 
We conduct a wide range of experiments on both synthetic and real-world datasets. The synthetic datasets are  PASCAL3D+~\cite{Xiang14-Pascal3DPlus} and FlyingThings3D~\cite{Mayer16CVPR-FT3D} and the real-world dataset is from 
%an autonomous driving benchmark dataset 
KITTI~\cite{Geiger13IJRR-KITTI}. 
We test the proposed approach against Sequential RANSAC~\cite{Torr98royalp-seqransac} and T-Linkage~\cite{Magri14CVPR-tlinkage}, and show it
% We also illustrate the comparison with algorithms from both optimization-based and clustering-based multi-model fitting methods, which are Sequential RANSAC~\cite{Torr98royalp-seqransac} and T-Linkage~\cite{Magri14CVPR-tlinkage} respectively. For some of the methods, a good initial clustering is crucial to maximize the performance. We thus consider the same method with different initial clustering as different baselines.
dominates these baselines on the multi-model 3D registration problem, and its performance is further improved by using SegmentAnything (SAM) \cite{Kirillov23arxiv-SAM} as initialization.

\subsection{Baselines and Initialization}

We compare our approach against T-Linkage~\cite{Magri14CVPR-tlinkage} and Sequential RANSAC (SRANSAC)~\cite{Torr98royalp-seqransac}. 
%T-Linkage is a clustering-based multi-model fitting algorithm, and SRANSAC is an optimization-based method. 
We also include a Naive baseline that applies Horn's method~\cite{Horn87josa} to compute a pose estimate for each initial cluster.

\myParagraph{T-Linkage~\cite{Magri14CVPR-tlinkage}} 
T-Linkage computes the distance between pairs of clusters and iteratively merges the closest pair of clusters. 
For each cluster $j$ (with associated pose $(\MR_j,\vt_j)$), T-Linkage defines a \emph{preference function} for point $i$ as
\begin{equation}
% \phi_{j, i} = \begin{cases}
%     \e^{- \|\vb_i - \MR_j \va_i - \vt\|/\tau_t} & d \leq 5 \tau \\
%     0 & d > 5 \tau \\
% \end{cases}.
\psi_{j, i} = \e^{- d_{j, i}/\tau_t} \text{ if } d_{j, i} \leq 5 \tau_t \text{ or } 0 \text{ otherwise},
\label{eq:preffunc}
\end{equation}
where $d_{j, i} := \|\vb_i \!-\! \MR_j \va_i \!-\! \vt_j\|$.
{It then uses the preference functions to compute distances between pairs of clusters, and terminates when the distance between every pair is large.
% become orthogonal for every pair of remaining clusters.
% computes the distance between two clusters using the Tanimoto distance,
% % builds on J-Linkage~\cite{Roberto08ECCV-jlinkage} and uses Tanimoto distance (instead of the Jaccard distance), 
% which is 0 when their preference functions are identical and 1 when they are orthogonal.
% The algorithm terminates when such functions become orthogonal for every pair of remaining clusters.
}
%  computes clusters' \emph{preference functions} and 
% The time constant $\tau_t$ represents the exponential decay rate in the preference function.
%  until no pair of clusters 
% %is similar to each other.
% %For each step, T-Linkage merges the most similar clusters 
% until all clusters' preference functions are orthogonal. 

\myParagraph{Sequential RANSAC~\cite{Torr98royalp-seqransac}} This baseline sequentially applies RANSAC and tries to recover one object at a time. After each RANSAC execution, the correspondences selected as inliers by RANSAC are used to compute a pose estimate and then removed to facilitate the search for other objects. 
% builds upon RANSAC that can robustly fit a single hypothesis with a large number of outliers. Each time we apply RANSAC on the point cloud, we obtain a hypothesis and the points associated with it. By removing these points from the point cloud and performing RANSAC repeatedly until the point cloud is empty, SRANSAC is able to recover multiple hypotheses.

\myParagraph{Initialization} SRANSAC does not require an initial guess for the clusters, while 
T-Linkage and our approach do.
In PASCAL3D+ we use Euclidean clustering on $\{\va_i\}_{i=1}^n$ to obtain initial clusters for both T-Linkage and EM.
In KITTI and FlyingThing3D, we ablate the effect of initial clustering, by initializing T-Linkage \cite{Magri14CVPR-tlinkage} and our method with SegmentAnything (SAM)~\cite{Kirillov23arxiv-SAM} or Euclidean clustering. We tune both initialization approaches to generate around 100 clusters.

% \bit
% \item Simulation experiments?
% \item Real tests?
% \eit

\subsection{Metrics}
We use three main performance metrics for evaluation. % to evaluate our approach against baselines. 
% To evaluate the performance of our algorithm compared with other baselines, we use three metrics that evaluate different aspects of the results.
% \begin{itemize}
%     \item 

\myParagraph{Per-Point Error ($\downarrow$)} 
This metric evaluates the average mismatch between the ground-truth and estimated point clouds associated with each object (including the background).
It first segments the first point cloud according to the ground-truth clusters 
to obtain $\va\at{i}, i=1,\ldots,M$, and then applies the ground-truth transformation to each object to obtain $\vb\at{i}, i=1,\ldots,M$. It repeats the same process using the estimated clusters and transforms to compute $\hat{\vb}\at{j}, j=1,\ldots,K$. 
Then, each estimated object $i$ is associated with the ground truth object $j$ that has the largest intersection with $i$ (\ie the largest number of points in common), 
and the Chamfer distance between $i$ and $j$ is recorded. The point error is defined as the average Chamfer distance across objects. 
% For each ground truth object $\vb\at{i}$ is selects the corresponding estimated object $\hat{\vb}\at{j}$ 
 % that has the smallest Chamfer distance for all $j=1,\ldots,m$, and calls the resulting distance $d_i$. Then the point error is the average error across objects, \ie $1 \ n \sum_i d_i$.
% in the point cloud $\va$ to compute the ``ground-truth'' point cloud $\vb^\star$. Moreover it computes a second point cloud $\hat{\vb}$ by applying the estimated transformation to $\va$. Then, for each object in the ground-truth 
% evaluates the average mismatch between the point cloud obtained by applying the ground-truth transformations to the 
% in the second point cloud $\vb$ by comparing the point cloud obtained by applying the ground-truth transformation 
%  between the point cloud after ground-truth transformation and after predicted transformation. 
%  The point error is defined as the average L2 distance (in meters) between each object in the point cloud masked over ground-truth masks.

\myParagraph{Rotation and Translation Error ($\downarrow$)} This metric evaluates the distance between the estimated and ground-truth poses. For each estimated object $H_j$, we find every ground-truth object $G_k$ that has a non-zero intersection with $H_j$. 
% 
% object with the largest intersection.
%we find all the corresponding groud-truth masks that intersect with the predicted mask. 
Then, we compute the \textit{translation error} as the Euclidean distance between the estimated and ground-truth object translation; 
the 
 % L2 distance between the inferred pose translation ($\mathbf{t}^{pred}$) and the ground-truth pose translation ($\mathbf{t}^{GT}$). 
 \textit{rotation error} is the angular distance~\cite{Hartley13ijcv} between the estimated  rotation and the ground truth rotation.
 %($\mathbf{R}^{pred}$) and the ground-truth rotation ($\mathbf{R}^{GT}$). 
 {The final translation and rotation errors of each estimated cluster are the weighted averages of the errors, where the weights are computed as ${|H_j \cap G_k| } / {|H_j|}$.}
 % the ratios of intersections between the estimated and the ground-truth object

 \myParagraph{Intersection over Union ($\uparrow$)} This metric evaluates the quality of the estimated clusters by assigning a ground-truth cluster to each estimated cluster with the largest intersection and calculating the average Intersection over Union (IoU). % over each pair of clusters.

% \end{itemize}

\input{tex/table1}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/icra24-results.pdf}
%     \caption{Results of 3 different metrics on two real datasets: FlyingThings3D and KITTI} 
%     \label{fig:boxplots-main}
% \end{figure*}
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/icra24-results-ft3d.pdf}
        \caption{FlyingThings3D Results}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/icra24-results-kit.pdf}
        \caption{KITTI Results}
        \label{fig:sub2}
    \end{subfigure}
    \caption{Results (IoU, per-point error, rotation error, and translation error) on (a) FlyingThings3D and (b) KITTI. We evaluate two variations of our method with two different initializations (SAM and Euclidean) and four baselines: Naive, Sequential RANSAC (SeqR), T-Linkage with SAM initialization (T-L (SAM)), and T-Linkage with Euclidean initialization (T-L (Euc.)).}
    \label{fig:boxplots-main}
\end{figure*}

% ===========================
\subsection{PASCAL3D+}
\myParagraph{Experimental Setup}
PASCAL3D+ \cite{Xiang14-Pascal3DPlus} is a synthetic dataset for 3D object understanding. We choose 7 objects from the dataset and downsample the vertices of their CAD models to form object point clouds (22,395 points overall). To generate point cloud pairs $\{(\va_i, \vb_i)\}_{i=1}^{n}$, we randomly sample 7 transformation matrices and apply them to each object point cloud. In this dataset, there are no outliers, and we want to test the capability of the compared techniques to tell the 7 objects apart and estimate their motion (Experiment 1).
% We thus have correspondences since $\vb$ is transformed from $\va$. 
We also repeat the same test in two more challenging settings, where we 
add zero-mean {Gaussian noise} with standard deviation $0.03$m to the point cloud $\{(\vb_i)\}_{i=1}^{n}$ (Experiment 2), and where ---in addition to the noise--- we 
assume 2 of the 7 objects have the same motion and we still want to tell them apart (Experiment 3).
We test our method with and without the distance term in{~\eqref{eq:likelihood}}; we denote the latter as ``Ours (Vanilla)''.
% Our algorithm with and without the distance term is tested.
We use Euclidean clustering (with 100 clusters) to obtain the initial clusters for Naive, T-Linkage, and our methods.
% and then apply the proposed EM algorithm. 
% We compare the predicted poses with the ground-truth poses, and the predicted clusters with the ground-truth masks. 
For our method, we set $\tau = 1.5$m, $m_\min = 4$, $T = 10$.
%The distance threshold $\tau$ for our method is 10, and 
We set $\tau_t = 0.2$m in T-Linkage. % is 2. 
For SRANSAC, we use 0.01m as the inlier threshold for experiment 1 (noiseless case) and 0.5m for the others and use 1000 max iterations.
Results are averaged over 100 runs.

\myParagraph{Results} 
Table~\ref{table:pascal3d} shows the results obtained with the compared techniques in the three settings described above. 
% We compare our method with T-Linkage \cite{Magri14CVPR-tlinkage} and Sequential RANSAC \cite{Torr98royalp-seqransac} for both cases with and without Gaussian additive noise. 
% Our method and T-Linkage use Euclidean clustering with 100 initial clusters as initialization while Sequential RANSAC has no initialization. In Table \ref{table:pascal3d}, 
In the noiseless case, SRANSAC and our methods achieve perfect scores (\ie errors are numerically zero). 
% This is because pose errors depend on the quality of cluster estimations, where our methods prevail.
% Our method and T-Linkage have similar pose errors, which are both numerically close to SRANSAC. However, since T-Linkage over-segments, it has a worse IoU. 
However, in the noisy experiments, our method outperforms other methods across metrics. This is because our method automatically adjusts the noise variance at each iteration and computes the likelihood function accordingly.
%takes the additive Gaussian noise into account in the likelihood function and . 
%In both Experiment 1 and Experiment 2, our methods perform similarly. 
% In Experiment 3, where we enforce two objects' motion to be identical, the lead of our method with the distance becomes even more evident. 
% With the distance term, our method can identify two objects that are relatively far apart even if they have the same motion. 
In Experiment 3, where we enforce two objects' motion to be identical, although both variants of our methods still estimate the poses with similar errors, the one with the distance term (``ours'') stands out in terms of IoU: with the distance term, our method can identify two objects that are relatively far apart even if they have the same motion. 
Naive reflects the quality of the initial clustering and typically leads to poor IoU. 
T-Linkage consistently improves over the initial clustering (Naive) in all experiments, but is not competitive with SRANSAC and our methods.
%has consistent improvement on the initial clustering in all three experiments.
% \LC{say that in the noiseless case, the pose errors are as good as T-Linkage, but T-linkage over-segments, leading to a worse IoU. explain why SRANSAC does not work in the noiseless case.}
% \LC{say the advantage of the proposed approach is even more evident in the noisy case-- note that so far vanilla and ours work pretty much the same.}
% \LC{the  comment on last experiment}
The runtime for SRANSAC is 30ms, while T-Linkage takes about 2s. Our method without the distance term takes about 800ms in Python on a Macbook Pro with M1 Pro chip. Adding the distance term in our method increases the runtime to a couple of seconds, since we have not optimized the distance computation.
%which is similar to T-linkage.
% Our method outperforms baselines in most metrics in both cases. Especially, when the additive noise exists, our method is still able to recover the hypothesis with low error and can correctly cluster point clouds almost perfectly. In Experiment 3, although pose and point errors are almost identical for both our methods, the one with \red{distance constraint} predicts better clusters since it is able to separate two objects even when they share the same hypothesis.



% ===========================
\subsection{FlyingThings3D}\label{sec:flying}
\myParagraph{Experimental Setup}
The FlyingThings3D \cite{Mayer16CVPR-FT3D} dataset has randomly moving objects from ShapeNet~\cite{Wu15cvpr-shapenets}. The dataset provides RGB images, segmentation masks, depth maps, and disparity maps. We construct the point clouds with ground-truth scene flows by back-projecting pixels to 3D points using disparity maps. 
%
In our method, to construct correspondences, we use the state-of-the-art scene flow model CamliRAFT~\cite{Liu22CVPR-camliflow} on RGB images and downsampled point cloud $\va$ with 32,768 points to get predicted scene flow $\vf$ and add predicted scene flow on the point cloud to get the next frame's point cloud $(\vb=\va + \vf)$. 
% We then use SegmentAnything (SAM) \cite{Kirillov23arxiv-SAM} to get the masks to initially cluster for our method. It is worth noting that while SAM is able to produce high-quality masks on images, the masks are always too fine-grained (for example, letters on a cereal box would be segmented as different clusters). Since we are interested in object-level masks, we use the fine-grained SAM masks to obatin  initialized clusters and use our method to merge them in terms of pose. Since every object in the dataset is moving, we can achieve object-level clustering with out method.
Using the object-level segmentation masks, we obtain ground-truth poses for each object cluster by running Horn's method on each object's point cloud and its counterpart displaced by the ground-truth scene flow.

We set the distance threshold in our method to be 5m, since the diameters of most objects are about 3m in the FlyingThings3D dataset. Then, for T-Linkage we set the constant $\tau_t$ to be 1m in \eqref{eq:preffunc}. For SRANSAC, we use 0.2 as the residual threshold and 1000 (maximum) iterations.

\myParagraph{Results}
We show the comparison between our method and other baselines on FlyingThings3D in Fig. \ref{fig:sub1}. As shown in the boxplots, our method outperforms other baselines. In particular, our method recovers the object clusters consistently (\ie it has the highest IoU) and works well with different kinds of initialization methods across all metrics. SRANSAC achieves a very low IoU score because it recovers over 50 clusters which is a lot more than the ground truth (about 10 clusters). T-Linkage clusters the point cloud better using Euclidean clustering which is considered as a weaker initialization method than SAM. This is because, in the FlyingThings3D dataset, since the objects are relatively far apart, the initial clusters from Euclidean clustering are significantly better than SAM. For our method, IoU scores are almost the same. This shows that our method is less sensitive to the quality of initial clustering. 
% We could tune SAM to generate a larger number of finer masks, but this will drastically increase the runtime of T-Linkage as it only removes one cluster at each step and needs to computer the similarity score between every two clusters.
% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/gray.eps} \vspace{-3mm}
%     \caption{
%         Boxplots for Flyingthings3d} \vspace{-5mm} 
%         \label{fig:coverfigure}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% ===========================
\subsection{KITTI}
\myParagraph{Experimental Setup}
The KITTI {\cite{Menze15cvpr-KITTIsceneflow,Geiger13IJRR-KITTI}} scene flow dataset consists of 400 {scenes} split into training, validation, and testing datasets with RGB images and depth. We only use the validation set because no ground-truth optical flow is provided in the testing set for us to evaluate. 
% \red{Note that none of the approaches we use are trained on this dataset, hence using the validation dataset is inconsequential. }

To run our method, we follow the same steps done for the FlyingThings3D dataset to construct correspondences and obtain initial clustering. 
% While KITTI does provide masks, the masks are at the category level, rather than instance level. For example, when multiple cars are in the scene, the cars will be separated from the background, but they will be clustered into one cluster representing all cars. 
Since KITTI only provides semantic masks, to compute ground truth poses and (instance-level) clusters we perform Euclidean clustering only on the point clouds with the car label in the ground-truth semantic segmentation and merge everything else as background, resulting in a masked point cloud with a cluster for each car and another cluster for the background. Then, we calculate the pose for each cluster, similar to FlyingThings3D. We use the same parameter choices as in Section~\ref{sec:flying} since the main moving objects here are cars which are also about 3m in length.

\myParagraph{Results}
In Fig. \ref{fig:sub2}, we compare our method and other baselines on the KITTI dataset. Our method outperforms other baselines. SRANSAC still suffers from over-segmenting as in the FlyingThings3D experiment. Since SAM performs better on KITTI (compared to Euclidean clustering), 
T-Linkage exhibits slightly better performance with the SAM initialization.
% Euclidean clustering could not give a better initial clustering than SAM on KITTI, T-Linkage now 
% recovers clusters of the point cloud better with the SAM initial clustering. 
% Note that CamLiRAFT produces higher quality scene flows \red{for the KITTI dataset as compared to the FlyingThings3D dataset as its KITTI model is fine-tuned on the FlyingThings model}. 
% Besides, SAM produces better segmentation masks since the RGB images in KITTI are less challenging to segment. This explains why the mask and error results for KITTI are overall better than those for FlyingThings3D despite KITTI being a real-world dataset.

% Compared to FlyingThings3D's results, the results on KITTI had fewer outliers and the effect of initial clustering is minimal. 
% \LC{I do not see much insights from the results here: why is SRANSAC failing? what is T-Linkage doing?}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \centering
% \begin{tabular}{l|l|c|c|c|c|c}
% \hline
% \multirow{2}{*}{Dataset}  &     \multirow{2}{*}{Method}             & Error per point & Pose rotation error & Pose translation error & Mask IoU & Overcounted Masks \\
%                         &                 & (meter) & (degree) & (meter) & (\%) & (\#) \\
% \hline
% \hline
% \multirow{3}{*}{PASCAL3D+} & Seq. RANSAC      &                 &                     &                        &  &    \\
%                            & T-Linkage        &                 &                     &            &            &     \\
%                            & Ours             &                 &                     &           &             &     \\
% \hline
% \multirow{5}{*}{FlyingThings3D}             & Seq. RANSAC      &                 &                     &                   &     &     \\
%                            & T-Linkage        &                 &                     &         &               &     \\
%                            & T-Linkage w/ SAM &                 &                     &          &              &     \\
%                            & EM               &                 &                     &           &             &     \\
%                            & Ours             &                 &                     &           &             &     \\

% \hline
% \multirow{5}{*}{KITTI}                       & Seq. RANSAC      &                 &                     &                  &      &   -  \\
%                            & T-Linkage        &                 &                     &          &              &    - \\
%                            & T-Linkage w/ SAM &                 &                     &            &            &   -  \\
%                            & EM               &                 &                     &            &            &  -   \\
%                            & Ours             &                 &                     &              &          &  -  \\
% \hline
% \end{tabular}
% \end{table*}
% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/gray.eps} \vspace{-3mm}
%     \caption{
%         Boxplots for KITTI} \vspace{-5mm} 
%         \label{fig:coverfigure}
% \end{figure}

==> tex/intro.tex <==
%!TEX root = ../main.tex
\section{Introduction}
\label{sec:intro}

3D registration is a foundational problem in robotics and computer vision and arises 
in several applications, including motion estimation and 
3D reconstruction~\cite{Henry12ijrr-rgbdMapping,Blais95pami-registration,Choi15cvpr-robustReconstruction, pan2022tax, pan2023tax},
object pose estimation~\cite{Drost10cvpr,Wong17iros-segicp,Zeng17icra-amazonChallenge, sim2019personalization, zhang2016health, zhang2020dex, zhang2021robots}, 
and medical imaging~\cite{Audette00mia-surveyMedical,Tam13tvcg-registrationSurvey, zhang2023flowbot++, teng2024gmkf};
rotation-only variations of the problem also arise in
panorama stitching~\cite{Bazin14eccv-robustRelRot, avigal20206, avigal2021avplug, elmquist2022art} and satellite attitude determination~\cite{wahba1965siam-wahbaProblem, shen2024diffclip, jin2024multi, yao2019recurrent}.  

\myParagraph{3D Registration}
In its simplest form, 3D registration looks for the rotation $\MR\in\SOthree$, the group of all rotations about the origin of $\mathbb{R}^3$ under the operation of composition, and translation $\vt\in\Real{3}$ that align two sets of points $\{\va_i\}_{i=1}^n$ and $\{\vb_i\}_{i=1}^n$. If the correspondences between the two sets of points are known, \ie we know that point $\vb_i$ in the second point cloud corresponds to point $\va_i$ in the first point cloud after a rigid transformation $(\MR,\vt)$ is applied, then the problem can be formulated as a nonlinear least squares problem and solved in closed form~\cite{Arun87pami,Horn87josa, devgon2020orienting, eisner2022flowbot3d, lim2021planar, lim2022real2sim2real}. More formally, if we assume the following generative model 
%relating vectors in the two sets of points
\beq
\label{eq:measModel1}
\vb_i = \MR \va_i + \vt + \vepsilon, \quad i=1,\ldots,n
\eeq
% \snote{\red{should we also have an index for} $\vepsilon$}
where $\vepsilon$ is a noise term distributed according to an isotropic Gaussian, then a maximum likelihood estimate for $(\MR, \vt)$ can be computed by solving the following nonlinear least squares:
\beq
\label{eq:estimator1} % \frac{1}{\sigma^2}
%(\MR^\star,\vt^\star) = \argmin
\min_{\MR\in\SOthree, \vt\in\Real{3}} \textstyle\sum_{i=1}^n \normsq{ \vb_i - \MR \va_i - \vt }{}
% \tag{REG}
\eeq
which admits a well-known closed-form solution via singular value decomposition (SVD)~\cite{Arun87pami,Horn87josa}.

\myParagraph{Robust 3D Registration} In practical problems, the measurements contain spurious correspondences. For instance, if the two point clouds represent two RGB-D scans at consecutive time stamps and we are trying to estimate the motion of the sensor between scans, we might attempt to establish correspondences $(\va_i,\vb_i)$, $i=1,\ldots,n$, using descriptor matching~\cite{Yang20tro-teaser}, optical flow~\cite{Barron94}, or scene flow~\cite{Vedula05pami-sceneFlow}.
As a result, some of the point pairs $(\va_i,\vb_i)$ may be well-approximated by the measurement model~\eqref{eq:measModel1}, while others are \emph{outliers} and largely deviate from~\eqref{eq:measModel1}, either because the pairs of points are incorrectly associated by the algorithm that establishes the correspondences, or because they do not lie on a static portion of the scene.
%on the object of interest.
This has motivated a large body of work on \emph{robust 3D registration}, which focuses on estimating $(\MR,\vt)$ in the face of outliers. In this case, the measurement model becomes:
\beq
\label{eq:measModel2}
\vb_i = \theta_i (\MR \va_i + \vt) + (1-\theta_i) \vo + \vepsilon, \quad i=1,\ldots,n
\eeq
where the (unknown) binary variable $\theta_i\in\{0,1\}$ decides whether $\vb_i$ is a rigid transformation of $\va_i$ (if $\theta_i=1$) or is an arbitrary vector $\vo$, independent of $(\MR,\vt)$ (if $\theta_i=0$). 
A plethora of works has attacked robust registration with outliers.
While we refer the reader to Section~\ref{sec:relatedWork} and~\cite{Yang20tro-teaser} for a more extensive discussion about related work, a popular approach is to resort to M-estimation, which attempts to compute an estimate for $(\MR, \vt)$ by minimizing a robust loss function. For instance, the work~\cite{Yang20tro-teaser} considers a truncated least squares loss:

\beq
\label{eq:estimator2}
% (\MR^\star,\vt^\star) = \hspace{-3mm}
\min_{ \substack{\MR\in\SOthree, \vt\in\Real{3}, \\ \theta_i \in \{0;1\}, i=1,\ldots,n}  } 
\textstyle\sum_{i=1}^n  \theta_i \normsq{ \vb_i - \MR \va_i - \vt }{} + (1-\theta_i) \bar{c}^2
% \tag{R-REG}
\eeq
which computes a least squares estimate for measurements with small residual errors (\ie whenever $\|\vb_i - \MR \va_i - \vt\|<\bar{c}$ the optimization forces $\theta_i=1$ and the second summand disappears), while discarding measurements with large residuals (when $\theta_i=0$, the objective becomes constant and the $i$-th measurement does not contribute to the estimate). 

\myParagraph{Multi-Model 3D Registration}
The robust registration problem~\eqref{eq:estimator2} looks for a single pose that explains the majority of  correspondences, while disregarding the others as outliers. 
In this paper, we ask: can we instead find further patterns in the outliers? 
or, in other words, can we \emph{simultaneously recover the motion of all 
objects present in the point clouds}?
% While the formulation fits many applications where one wants to recover a single pose (\eg the pose of a moving sensor, or a single object) it has two drawbacks. First, it is doomed to fail in the presence of a large number of adversarial outliers~\cite{Carlone23fnt-estimationContracts}. Second, it disregards all measurements that do not agree with the best pose estimate as outliers, without attempting to detect further patterns in the outliers (\eg these might correspond to other moving objects in the robot's surroundings). 
% In this paper, we generalize the robust registration problem by attempting to \emph{simultaneously recover the motion of all objects present in the point clouds}. 
More formally, we assume the following generative model: 
\beq
\label{eq:measModel3}
\vb_i = \textstyle\sum_{j=1}^\nrModels \theta_{i,j} (\MR_j \va_i + \vt_j) + \theta_{i,0} \; \vo + \vepsilon, \quad i=1,\ldots,n
% \tag{M-REG}
\eeq
where for each measurement $i$, the vector $\vtheta_i = [\theta_{i,0} \; \theta_{i,1} \; \ldots \theta_{i,\nrModels}] \in \{0;1\}^{\nrModels+1}$  is an unknown binary vector with a single entry equal to 1, $\nrModels$ it the number of objects (unknown a priori), and $(\MR_j,\vt_j)$ is the motion of the $j$-th object, for $j=1,\ldots,\nrModels$. In words, each point $\vb_i$ in~\eqref{eq:measModel3} is either generated by an object $j$ (if $\theta_{i,j}=1$ for a $j\in\{1,\ldots,\nrModels\}$) or is an outlier (if $\theta_{i,0}=1$). 
Clearly, when $\nrModels=1$, eq.~\eqref{eq:measModel3} falls back to the  robust registration setup in~\eqref{eq:measModel2}. 

\myParagraph{Contribution}
An algorithm based on Expectation-Maximization was recently proposed in \cite{jin2024multimodel} to solve the multi-model 3D registration problem described above. Despite its outstanding experimental results, the paper did not theoretically justify the conditions under which the EM approach converges to the ground truth. In this project, we aim to close this gap by establishing such conditions. By taking advantage of the probabilistic tail bounds developed throughout the course, we provide detailed theoretical analysis of the algorithm. As a consequence, our result suggests that the EM scheme converges to the ground truth as long as the initialization of the vectors $\vtheta_i$ is sufficient to capture all objects of interest. %, despite the presence of outliers. 
%  We evaluate the EM scheme in simulated and real datasets ranging from table-top 
% scenes to large self-driving scenarios (Fig.~\ref{fig:coverfigure}) and demonstrate its effectiveness when combined with state-of-the-art 
% %learning-based 
% scene flow methods %(CamliRAFT~\cite{Liu22CVPR-camliflow}) 
% to establish dense correspondences.  

==> tex/problemFormulation.tex <==
%!TEX root = ../main.tex

\section{Problem Formulation}
\label{sec:problemFormulation}

\LC{Luca will take a stab at this}


==> tex/qual.tex <==
\section{Qualitative Results}

In this section, we show two examples (\cref{fig:coverfigure}) of the algorithm proposed in \cite{jin2024multimodel} on the real-world autonomous driving dataset.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/icra2024-teaser.pdf}
    \caption{Our algorithm aims to recover the motion of all objects (and background) in a scene from point cloud observations. The figure reports two results produced by our approach on the KITTI dataset.
    % Two examples of the proposed methods segmenting point clouds from the KITTI dataset. In the top example, since the points are sampled sparsely, the white car on the left did not get sampled sufficiently, so it was not clustered. 
    \label{fig:coverfigure}}
\end{figure}

==> tex/relatedWork-long2.tex <==
%!TEX root = ../main.tex
\section{Related work}
\label{sec:relatedWork}

% \LC{David: assign writing tasks for each paragraph}
\myParagraph{Robust Estimation in Robotics and Vision}
We refer the reader to~\cite{Yang20tro-teaser} for an extensive review of robust 3D registration and to~\cite{Carlone23fnt-estimationContracts,Bosse17fnt} for a broader overview of robust estimation in robotics and vision.
 % While we refer the reader to~\cite{Yang20tro-teaser} for an extensive review of robust 3D registration, 
 % Here we briefly mention three main classes of approaches for robust estimation: 
 % M-estimation, consensus maximization, and graph-theoretic outlier pruning. 
\emph{M-estimation} is a popular framework for robust estimation and formulates the estimation problem as an optimization problem with a robust loss function that is designed to mitigate the influence of outliers.   
The resulting problem is typically optimized using iterative local solvers~\cite{MacTavish15crv-robustEstimation}, heuristics to improve global convergence (\eg \emph{graduated non-convexity}~\cite{Blake1987book-visualReconstruction,Black96ijcv-unification,Zhou16eccv-fastGlobalRegistration,Yang20ral-GNC,Antonante21tro-outlierRobustEstimation}), or 
certifiably optimal algorithms (\cite{Yang22pami-certifiablePerception} and the references therein).
% , or \BnB~\cite{Enqvist08eccv-robustOptimalPose}.
\emph{Consensus Maximization} is a related framework that 
is a framework for robust estimation that aims to find {the largest} set of measurements with errors {below} a user-defined threshold.
Consensus maximization is NP-hard~\cite{Chin18eccv-robustFitting,Antonante21tro-outlierRobustEstimation},
hence the community has resorted to randomized approaches, such as RANSAC~\cite{Fischler81}.
%, which repeatedly draws a minimal
%subset of measurements and loo. %, has been the dominating approach.
RANSAC repeatedly draws a minimal subset of measurements from which a rough estimate is computed,
and the algorithm stops after finding an estimate that agrees with a large set of measurements.
% \omitted{At each iteration, RANSAC randomly draws a minimal subset of measurements from which a rough estimate is computed,
% and the algorithm stops after finding an estimate that agrees with a large set of measurements.}
While RANSAC works well for problems where the minimal set is small and there are not many outliers,
the average number of iterations it requires %to find the inliers %a \HYedit{consensus set}
increases exponentially with the percentage of outliers~\cite{Raguram08-RANSACcomparative}, making it impractical for problems with many outliers.
%  of samples necessary for a minimal solver to solve the estimation problem.
% For each estimate, a corresponding consensus set is obtained and the estimate with the largest consensus set is returned.
% While RANSAC and its variants \cite{Torr00cviu,Chum03-LORANSAC,Barath18-graphCutRANSAC} have been the dominating approaches for geometric estimation,
% they cannot garantee that the obtained solution is globally optimal.
On the other hand, global solvers, such as branch-and-bound (\BnB)~\cite{Li09cvpr-robustFitting} and tree search~\cite{Cai19ICCV-CMtreeSearch}, exist but scale poorly with the problem size, with \BnB being exponential in the size of $\vxx$, and tree search being exponential in the number of outliers~\cite{Cai19ICCV-CMtreeSearch}.


Robust estimation is a very dynamic and active research area in vision and robotics~\cite{Peng23CVPR-IRLS,Barik23arxiv-invexity,Carlone23fnt-estimationContracts}.


% TODO: Reivew hypergraph stuff
{\bf Graph-based Outlier pruning methods} aim at discarding gross outliers from the set of measurements. 
These methods do not necessarily reject all the outliers, hence they are often used as a preprocessing for
 M-estimation or maximum consensus~\cite{Yang20tro-teaser,Shi21icra-robin}.
% Alternatively,
% {\bf graph-based methods}
% form another viable option for \JS{solving the consensus maximization problem approximately}.
Outlier pruning methods detect outliers by analyzing a
% These methods usually first formulate the consensus maximization problem as a 
\emph{compatibility graph},
where vertices represent data points and
edges represent pre-defined compatibility measures between data points~\cite{Shi21icra-robin}.
% Consensus maximization can then be solved through a graph-theoretic lens.
Bailey\setal~\cite{Bailey00icra-dataAssociation}~propose a Maximum Common Subgraph algorithm for feature matching in lidar scans.
Segundo and Artieda~\cite{San15-cliqueFeatureMatching} build an association graph and find the maximum clique for 2D image feature matching.
Perera and Barnes~\cite{Perera12-maxCliqueSegmentation} segment objects under rigid body motion with a clique formulation.
Leordeanu and Hebert~\cite{Leordeanu05-spectral} {establish image matches by finding strongly-connected clusters in the correspondence graph with an approximate spectral method.}
Enqvist~\etal~\cite{Enqvist09iccv} develop an outlier rejection algorithm for 3D-3D and 2D-3D registration based on approximate vertex cover. %; the resulting solver can only handle small problems~\cite{Parra19arXiv-practicalMaxClique}.
Recent progress in graph algorithms (\eg~\cite{Rossi15parallel, Parra19arXiv-practicalMaxClique})
has led to fast graph-theoretic outlier pruning algorithms that are robust to 
 extreme outlier rates, see, \eg~\cite{Yang20tro-teaser}.
% a convergence between fast implementations and robust solvers,
% such as \teaserpp~\cite{Yang20tro-teaser}, that are robust to high-noise and outliers.


\myParagraph{List-Decodable Regression}
%INTRO 
Classical robust statistics has focused on the problem of recovering
signals from a \emph{minority} of the data being corrupted. 
Recently there has been an increased focus on the setting where a \emph{majority} of the samples are corrupted (see, for e.g. \cite{Charikar17stoc-robustEstimationTheory,Karmalkar19neurips-ListDecodableRegression, Raghavendra20soda-ListDecodableRegressions,diakonikolas2020list,cherapanamjeri2020list}).
While returning a single accurate hypothesis in this regime is information-theoretically impossible, 
one may be able to compute a small list of hypotheses with the guarantee that at least one of them is accurate.
This relaxed notion is called \emph{list-decodable} learning.

In this line of work, the problem most relevant to the one we study is the problem of list-decodable regression was first studied in \cite{Karmalkar19neurips-ListDecodableRegression} and \cite{Raghavendra20soda-ListDecodableRegressions}, 
where, for a small constant ($\alpha$) fraction of inliers, they demonstrated polynomial-time algorithms to perform list-decodeable linear regression. 
Subsequent work has shown that an exponential dependence on $1/\alpha$ is necessary for a large class of algorithms \cite{diakonikolas2021statistical}. 
These papers assume that the inliners come from gaussian measurements of an unknown signal vector. 
However, this assumption is not valid in several real-world settings.
Since the problem of list-decodable linear regression is a generalization of the problem of \emph{mixed} linear regression (defined later),
it turns out that the same algorithm from \cite{Karmalkar19neurips-ListDecodableRegression} is also very amenable to problems of perception such as the single-hypothesis Wabha problem as shown in \cite{Carlone23fnt-estimationContracts}. 
\snote{Prev paper not scalable. 
list-decodable reg paper used for multi-modal rot estimation}

% related 

% Sushrut's work

% others..

% Estimation Constrats: use list-decodable to recover multiple structures..

\myParagraph{Multi-model Fitting in Computer Vision} Early work in computer vision has studied the problem of simultaneously recovering multiple models from noisy measurements. In the realm of multi-model fitting, two primary research directions dominate: clustering-based methods and optimization-based techniques. Clustering-based methods have a variety of methods including but not limited to hierarchical clustering~\cite{Magri14CVPR-tlinkage}, \cite{Roberto08ECCV-jlinkage}, kernel fitting~\cite{Chin09ICCV-statlearning}, \cite{Chin10CRPR-kerneloptim}, matrix factorization~\cite{Magri17IVC-RPA}, \cite{Mariano17CVPR-NMU} and hypergraph partitioning~\cite{Lin19AAAI-hypermultifitting}, \cite{Purkait17TPAMI-clusterhypergraph}. On the optimization-based front, consensus-based approaches are popular. Techniques like Sequential RANSAC~\cite{Torr98royalp-seqransac}, Multi-RANSAC~\cite{Zuliani05ICIP-multiransac}, and RANSACOV~\cite{Magri16CVPR-ransacov} focus on maximizing the consensus among the data points, providing a statistical framework that is robust to noise and outliers. Refined methods such as Pearl~\cite{Isack12IJCV-pearl} and Progressive-x~\cite{Daniel19ICCV-progx} go a step further by incorporating additional priors into the objective function, thereby providing more nuanced fitting solutions that can leverage extra constraints or specialized information.

% aim to recursively break down the data into smaller clusters, making it easier to fit individual models. Kernel fitting techniques take a slightly different approach by using Kernel Density Estimation (KDE) to model the distribution of data points, which is particularly effective for non-linear underlying models.

% Robust Matrix Factorization is another clustering-based strategy that decomposes the data into lower-dimensional matrices. This not only simplifies the computational burden but also tends to enhance the quality of model fitting by isolating noise and outliers. Other advanced clustering techniques like biclustering and hypergraph partitioning have also been explored to capture complex relationships among data points.


% TJ ..
% While multi-structure fitting is very close to the problem we consider in this paper, ...
% differences, and novel contributions. 

\myParagraph{Mixture of Linear Regression in Applied Mathematics} 
In the problem of learning a mixture of linear regressions, 
each observation is generated from one of the several unknown linear regression components, 
where the identity of the generated component is also unknown.
Unfortunately, the task of recovering the linear signals from this data is NP hard in general \cite{yi2014alternating}. 
However, under certain assumptions on the underlying distribution (e.g., $x$ of different components all from the standard Gaussian, or only 2 components),
Several approaches have been studied for this problem -- 
including algorithms based on the method of moments \cite{sedghi2016provable,li2018learning}, 
alternating-minimization \cite{yi2014alternating,YiCS16} and 
Expectation-Maximization \cite{FariaSoromenho10,KYB19}. 
This setting has also been used as a benchmark algorithms for nonconvex optimization
\cite{chaganty2013spectral,KYB19}
In contrast to prior work, we do not make the Gaussian assumption on the measurements. 
In our case our variables lie on a manifold and our setup is more specific
to the problem setting we consider.
(See \Cref{sec:theory} for more details). 

\myParagraph{Learning-based Methods for Motion Tracking} Optical flow methods~\cite{Teed21ECCV-raft}, \cite{Ilg16arxiv-flownet2} which estimate the pixel movements between two video frames can segment moving objects from the videos but are not able to leverage 3D information. Scene flow from RGB-D Frames is concerned with the problem of estimating dense 3D motion for each pixel from a pair of stereo or RGB-D frames. Recent approaches such as DRISF~\cite{Ma19CVPR-drisf} and RigidMask~\cite{Yang21CVPR-rigidmask}, divide scene flow estimation into multiple subtasks and build modular networks comprising one or more submodules for each subtask. 
% Traditional methods like those cited in studies utilize variational and discrete optimization, treating scene flow as an energy minimization problem. In contrast,
% While DRISF estimates optical flow, depth, and segmentation from two consecutive stereo images and employs a Gaussian-Newton solver to find the best 3D rigid motion, RigidMask predicts segmentation masks for the background and multiple rigidly moving objects, which are then parameterized by 3D rigid transformation. 
% Although these methods have shown significant progress, their submodules operate independently, failing to e
Exploiting different modalities, RAFT-3D~\cite{Teed21CVPR-raft3d} attempts to address this by using feature-level fusion, but its early fusion of images and depth maps to RGB-D frames makes it challenging for 2D CNNs to take advantage of 3D structural information. CamLiRAFT~\cite{Liu22CVPR-camliflow}, \cite{Liu23arxiv-camliraft} proposes a multi-stage bi-directional pipeline to better fusion multi-modal information so that it can both process images for optical flows and directly extract feature from points for scene flows without suffering from the loss due to voxelization or projection.

% Turning to scene flow from point clouds, PointNet~\cite{} is a pioneering framework for studying deep learning on point sets, processing 3D points directly, often sourced from LiDAR. Various researchers have explored point-based approaches to scene flow estimation. For instance, FlowNet3D builds on PointNet++ and uses a flow embedding layer to represent the motion of points. FlowNet3D++ enhances performance by adding geometric constraints, whereas HPLFlowNet employs permutohedral lattice projection inspired by Bilateral Convolutional Layers. 


% Other approaches like PointPWCNet introduce a learnable cost volume for point clouds, FLOT considers the problem as graph matching between corresponding points in adjacent frames, and PV-RAFT and FlowStep3D capture both local and long-range dependencies of point pairs through point-voxel correlation fields and a recurrent architecture, respectively. However, similar to their counterparts in RGB-D scene flow, these point-cloud-based methods also fail to exploit color features provided by images, thus limiting their performance.

% RigidMask:
% \url{https://arxiv.org/pdf/2101.03694.pdf}

% RAFT \\
% RAFT3D \\
% CAMLIRAFT \\

% \url{https://ieeexplore.ieee.org/document/5459150}




==> tex/relatedWork.tex <==
%!TEX root = ../main.tex
\section{Related work}
\label{sec:relatedWork}

% \LC{David: assign writing tasks for each paragraph}
\myParagraph{Robust Estimation in Robotics and Vision}
Robust estimation is an active research area in robotics and vision~\cite{Peng23CVPR-IRLS,Barik23arxiv-invexity,Carlone23fnt-estimationContracts} and has been attacked using different frameworks, including M-estimation~\cite{MacTavish15crv-robustEstimation,Black96ijcv-unification,Yang20ral-GNC,Yang22pami-certifiablePerception}, 
consensus maximization~\cite{Chin18eccv-robustFitting,Antonante21tro-outlierRobustEstimation} (typically solved using sampling-based algorithms, such as RANSAC~\cite{Fischler81}), or graph-theoretic  methods~\cite{Yang20tro-teaser,Shi21icra-robin,Parra19arXiv-practicalMaxClique,Enqvist09iccv}.
We refer the reader to~\cite{Yang20tro-teaser} for an extensive review of robust 3D registration and to~\cite{Carlone23fnt-estimationContracts,Bosse17fnt} for an overview of robust estimation across robotics and vision.
 % While we refer the reader to~\cite{Yang20tro-teaser} for an extensive review of robust 3D registration, 
 % Here we briefly mention three main classes of approaches for robust estimation: 
 % M-estimation, consensus maximization, and graph-theoretic outlier pruning. 
% \emph{M-estimation} is a popular framework for robust estimation and formulates the estimation problem as an optimization problem with a robust loss function that is designed to mitigate the influence of outliers.   
% The resulting problem is typically optimized using iterative local solvers~\cite{MacTavish15crv-robustEstimation}, heuristics to improve global convergence (\eg \emph{graduated non-convexity}~\cite{Blake1987book-visualReconstruction,Black96ijcv-unification,Zhou16eccv-fastGlobalRegistration,Yang20ral-GNC,Antonante21tro-outlierRobustEstimation}), or 
% certifiably optimal algorithms (\cite{Yang22pami-certifiablePerception} and the references therein).
% % , or \BnB~\cite{Enqvist08eccv-robustOptimalPose}.
% \emph{Consensus Maximization} is a related framework that 
% is a framework for robust estimation that aims to find {the largest} set of measurements with errors {below} a user-defined threshold.
% Consensus maximization is NP-hard~\cite{Chin18eccv-robustFitting,Antonante21tro-outlierRobustEstimation},
% hence the community has resorted to randomized approaches, such as RANSAC~\cite{Fischler81}.
% %, which repeatedly draws a minimal
% %subset of measurements and loo. %, has been the dominating approach.
% RANSAC repeatedly draws a minimal subset of measurements from which a rough estimate is computed,
% and the algorithm stops after finding an estimate that agrees with a large set of measurements.
% % \omitted{At each iteration, RANSAC randomly draws a minimal subset of measurements from which a rough estimate is computed,
% % and the algorithm stops after finding an estimate that agrees with a large set of measurements.}
% While RANSAC works well for problems where the minimal set is small and there are not many outliers,
% the average number of iterations it requires %to find the inliers %a \HYedit{consensus set}
% increases exponentially with the percentage of outliers~\cite{Raguram08-RANSACcomparative}, making it impractical for problems with many outliers.
%  of samples necessary for a minimal solver to solve the estimation problem.
% For each estimate, a corresponding consensus set is obtained and the estimate with the largest consensus set is returned.
% While RANSAC and its variants \cite{Torr00cviu,Chum03-LORANSAC,Barath18-graphCutRANSAC} have been the dominating approaches for geometric estimation,
% they cannot garantee that the obtained solution is globally optimal.
% On the other hand, global solvers, such as branch-and-bound (\BnB)~\cite{Li09cvpr-robustFitting} and tree search~\cite{Cai19ICCV-CMtreeSearch}, exist but scale poorly with the problem size, with \BnB being exponential in the size of $\vxx$, and tree search being exponential in the number of outliers~\cite{Cai19ICCV-CMtreeSearch}.
% TODO: Reivew hypergraph stuff
% {\bf Graph-based Outlier pruning methods} aim at discarding gross outliers from the set of measurements. 
% These methods do not necessarily reject all the outliers, hence they are often used as a preprocessing for
%  M-estimation or maximum consensus~\cite{Yang20tro-teaser,Shi21icra-robin}.
% % Alternatively,
% % {\bf graph-based methods}
% % form another viable option for \JS{solving the consensus maximization problem approximately}.
% Outlier pruning methods detect outliers by analyzing a
% % These methods usually first formulate the consensus maximization problem as a 
% \emph{compatibility graph},
% where vertices represent data points and
% edges represent pre-defined compatibility measures between data points~\cite{Shi21icra-robin}.
% % Consensus maximization can then be solved through a graph-theoretic lens.
% Bailey\setal~\cite{Bailey00icra-dataAssociation}~propose a Maximum Common Subgraph algorithm for feature matching in lidar scans.
% Segundo and Artieda~\cite{San15-cliqueFeatureMatching} build an association graph and find the maximum clique for 2D image feature matching.
% Perera and Barnes~\cite{Perera12-maxCliqueSegmentation} segment objects under rigid body motion with a clique formulation.
% Leordeanu and Hebert~\cite{Leordeanu05-spectral} {establish image matches by finding strongly-connected clusters in the correspondence graph with an approximate spectral method.}
% Enqvist~\etal~\cite{Enqvist09iccv} develop an outlier rejection algorithm for 3D-3D and 2D-3D registration based on approximate vertex cover. %; the resulting solver can only handle small problems~\cite{Parra19arXiv-practicalMaxClique}.
% Recent progress in graph algorithms (\eg~\cite{Rossi15parallel, Parra19arXiv-practicalMaxClique})
% has led to fast graph-theoretic outlier pruning algorithms that are robust to 
%  extreme outlier rates, see, \eg~\cite{Yang20tro-teaser}.
% a convergence between fast implementations and robust solvers,
% such as \teaserpp~\cite{Yang20tro-teaser}, that are robust to high-noise and outliers.


\myParagraph{List-Decodable Regression}
%INTRO 
While standard robust estimation computes an estimate that agrees with the majority of the measurements, 
recent work in robust statistics has focused on recovering an estimate from a handful of inliers hidden among an overwhelming amount of outliers, \eg~\cite{Charikar17stoc-robustEstimationTheory,Karmalkar19neurips-ListDecodableRegression, Raghavendra20soda-ListDecodableRegressions,diakonikolas2020list,cherapanamjeri2020list}. In this regime, returning a  
% Classical robust statistics has focused on the problem of recovering
% signals from a \emph{minority} of the data being corrupted. 
% Recently there has been an increased focus on the setting where a \emph{majority} of the samples are corrupted (see, for e.g. \cite{Charikar17stoc-robustEstimationTheory,Karmalkar19neurips-ListDecodableRegression, Raghavendra20soda-ListDecodableRegressions,diakonikolas2020list,cherapanamjeri2020list}).
% While returning a 
single accurate hypothesis is information-theoretically impossible, 
and one has to compute a list of hypotheses to guarantee that at least one of them is accurate.
This setup, typically referred to as \emph{list-decodable} regression, 
% This relaxed notion is called \emph{list-decodable} learning.
% In this line of work, the problem most relevant to the one we study is the problem of list-decodable regression 
was first studied in \cite{Karmalkar19neurips-ListDecodableRegression} and~\cite{Raghavendra20soda-ListDecodableRegressions}, which proposed and analyzed algorithms based on semidefinite relaxations. The work~\cite{Carlone23fnt-estimationContracts} observes that the algorithm in~\cite{Karmalkar19neurips-ListDecodableRegression} can be easily adapted to solve a multi-model rotation-only registration problem; however, the resulting relaxation is impractically slow (\eg 3 minutes to solve a problem with 50 measurements).
% where, for a small constant ($\alpha$) fraction of inliers, they demonstrated polynomial-time algorithms to perform list-decodeable linear regression. 
% Subsequent work has shown that an exponential dependence on $1/\alpha$ is necessary for a large class of algorithms \cite{diakonikolas2021statistical}. 
% These papers assume that the inliners come from gaussian measurements of an unknown signal vector. 
% However, this assumption is not valid in several real-world settings.
% Since the problem of list-decodable linear regression is a generalization of the problem of \emph{mixed} linear regression (defined later),
% it turns out that the same algorithm from \cite{Karmalkar19neurips-ListDecodableRegression} is also very amenable to problems of perception such as the single-hypothesis Wabha problem as shown in \cite{Carlone23fnt-estimationContracts}. 
% \snote{Prev paper not scalable. 
% list-decodable reg paper used for multi-modal rot estimation}
% related 
% Sushrut's work
% others..
% Estimation Constrats: use list-decodable to recover multiple structures..

\myParagraph{Multi-Model Fitting in Computer Vision} Early work in computer vision has studied the problem of simultaneously recovering multiple models from noisy measurements. 
The corresponding literature includes clustering-based and optimization-based methods.
% In the realm of multi-model fitting, two primary research directions dominate: clustering-based methods and optimization-based techniques. 
Clustering-based methods span a variety of techniques, including  hierarchical clustering~\cite{Magri14CVPR-tlinkage}, \cite{Roberto08ECCV-jlinkage}, kernel fitting~\cite{Chin09ICCV-statlearning}, \cite{Chin10CRPR-kerneloptim}, matrix factorization~\cite{Magri17IVC-RPA}, \cite{Mariano17CVPR-NMU} and hypergraph partitioning~\cite{Lin19AAAI-hypermultifitting}, \cite{Purkait17TPAMI-clusterhypergraph}. 
Optimization-based methods include generalizations of RANSAC to the multi-model setup, including 
%focus on variants of the consen
% On the optimization-based front, consensus-based approaches are popular. Techniques like 
Sequential RANSAC~\cite{Torr98royalp-seqransac}, Multi-RANSAC~\cite{Zuliani05ICIP-multiransac}, and RANSACOV~\cite{Magri16CVPR-ransacov}.
 % focus on maximizing the consensus among the data points, providing a statistical framework that is robust to noise and outliers. 
 Other methods such as Pearl~\cite{Isack12IJCV-pearl} and Progressive-X~\cite{Daniel19ICCV-progx} {take a step further by incorporating additional priors into the objective function.}
 %, thereby providing more nuanced fitting solutions that can leverage extra constraints or specialized information.
%
% aim to recursively break down the data into smaller clusters, making it easier to fit individual models. Kernel fitting techniques take a slightly different approach by using Kernel Density Estimation (KDE) to model the distribution of data points, which is particularly effective for non-linear underlying models.
%
% Robust Matrix Factorization is another clustering-based strategy that decomposes the data into lower-dimensional matrices. This not only simplifies the computational burden but also tends to enhance the quality of model fitting by isolating noise and outliers. Other advanced clustering techniques like biclustering and hypergraph partitioning have also been explored to capture complex relationships among data points.
%
% TJ ..
% While multi-structure fitting is very close to the problem we consider in this paper, ...
% differences, and novel contributions. 

\myParagraph{Mixture of Linear Regression in Applied Mathematics} 
In the problem of learning a mixture of linear regressions, 
each measurement is generated from one of several unknown linear regression components, 
and one has to associate measurements to components and estimate the components.
% regressinwhere the identity of the generated component is also unknown.
% Unfortunately, the task of recovering the linear signals from this data is 
This problem is known to be NP hard in general~\cite{yi2014alternating}. 
However, under certain assumptions on the underlying distribution (\eg the regressors follow a standard Gaussian distribution, or there are only two mixture components),
several approaches have successfully tackled the problem,
including algorithms based on the method of moments \cite{sedghi2016provable,li2018learning}, 
alternating-minimization \cite{yi2014alternating,YiCS16}, and 
Expectation-Maximization \cite{FariaSoromenho10,KYB19,kwon20aistats-EM-MLR}. 
% This setting has also been used as a benchmark algorithms for nonconvex optimization
% \cite{chaganty2013spectral,KYB19}
Contrary to this line of work, in this paper we do not make a Gaussian assumption on the regressors, 
and we consider a 3D registration problem % b(where variables live on a manifold) 
rather than a linear regression setup.
%our variables live on a manifold (\ie they are 3D poses) rather than 
% In contrast to prior work, we do not make the Gaussian assumption on the measurements. 
% In our case our variables lie on a manifold and our setup is more specific
% to the problem setting we consider.
% (See \Cref{sec:theory} for more details). 

\myParagraph{Learning-based Methods for Motion Tracking} 
Learning-based methods have recently demonstrated excellent performance in 2D and 3D motion tracking.
Optical flow methods~\cite{Teed21ECCV-raft,Ilg16arxiv-flownet2} estimate the pixel displacement between two  frames, which can be used to segment moving objects from a video. 
Scene flow estimates dense 3D motion for each pixel from a pair of stereo or RGB-D frames. Other approaches, such as DRISF~\cite{Ma19CVPR-drisf} and RigidMask~\cite{Yang21CVPR-rigidmask}, divide scene flow estimation into multiple subtasks and build modular networks to solve each subtask.
%comprising one or more submodules for each subtask. 
% Traditional methods like those cited in studies utilize variational and discrete optimization, treating scene flow as an energy minimization problem. In contrast,
% While DRISF estimates optical flow, depth, and segmentation from two consecutive stereo images and employs a Gaussian-Newton solver to find the best 3D rigid motion, RigidMask predicts segmentation masks for the background and multiple rigidly moving objects, which are then parameterized by 3D rigid transformation. 
% Although these methods have shown significant progress, their submodules operate independently, failing to e
% Exploiting different modalities, 
RAFT-3D~\cite{Teed21CVPR-raft3d} computes the scene flow by using feature-level fusion.
% but its early fusion of images and depth maps to RGB-D frames makes it challenging for 2D CNNs to take advantage of 3D structural information. 
CamLiRAFT~\cite{Liu22CVPR-camliflow,Liu23arxiv-camliraft} proposes a multi-stage pipeline to better fuse multi-modal information without suffering from accuracy loss due to voxelization.
% so that it can both process images for optical flows and directly extract feature from points for scene flows without suffering from the loss due to voxelization or projection.

% Turning to scene flow from point clouds, PointNet~\cite{} is a pioneering framework for studying deep learning on point sets, processing 3D points directly, often sourced from LiDAR. Various researchers have explored point-based approaches to scene flow estimation. For instance, FlowNet3D builds on PointNet++ and uses a flow embedding layer to represent the motion of points. FlowNet3D++ enhances performance by adding geometric constraints, whereas HPLFlowNet employs permutohedral lattice projection inspired by Bilateral Convolutional Layers. 


% Other approaches like PointPWCNet introduce a learnable cost volume for point clouds, FLOT considers the problem as graph matching between corresponding points in adjacent frames, and PV-RAFT and FlowStep3D capture both local and long-range dependencies of point pairs through point-voxel correlation fields and a recurrent architecture, respectively. However, similar to their counterparts in RGB-D scene flow, these point-cloud-based methods also fail to exploit color features provided by images, thus limiting their performance.

% RigidMask:
% \url{https://arxiv.org/pdf/2101.03694.pdf}

% RAFT \\
% RAFT3D \\
% CAMLIRAFT \\

% \url{https://ieeexplore.ieee.org/document/5459150}




==> tex/table1.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
\caption{Results for synthetic PASCAL3D+ dataset. Experiment 1: Noiseless. Experiment 2: with additive Gaussian noise. Experiment 3: with additive Gaussian noise and 2 objects with the same motion.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l}
\hline
                    & Metric & \multicolumn{5}{c}{Method}    \\
\cline{3-7}
                    & (Mean) & Naive & SRANSAC & T-Linkage   & Ours (Vanilla) & Ours \\
\hline
\hline
\multirow{4}{*}{1}  & Per-point Error [m]    &   0.0454 & \textbf{9.56e-15} &  0.163 &  \textbf{9.56e-15} & \textbf{9.56e-15}    \\
                    & Rotation error [deg]     &   46.8 & \textbf{8.69e-7} & 19.6 &  \textbf{8.69e-7} &  \textbf{8.69e-7}    \\
                    & Translation error [m]  &   0.487 & \textbf{3.81e-15} & 0.242 & \textbf{3.81e-15} & \textbf{3.81e-15}    \\
                    & IoU                &   0.698 & \textbf{1.0} & 0.723 & \textbf{1.0}  & \textbf{1.0}     \\
\hline
\multirow{4}{*}{2}  & Per-point Error [m]   &   0.0550 & 0.332 & 0.199 & 0.0135 &  \textbf{0.00516}     \\
                    & Rotation error [deg]    &   81.6 & 74.2 &  27.6 & 2.42 & \textbf{1.53}    \\
                    & Translation error [m]  &   0.858  & 0.796 & 0.287 & 0.0286 & \textbf{0.0165}   \\
                    & IoU                &    0.668 & 0.450 & 0.785 & 0.908 & \textbf{0.964}    \\ 
\hline
\multirow{4}{*}{3}  & Per-point Error [m]    & 0.0104 & 0.321 & 0.215 &  0.00860 & \textbf{0.00776}   \\
                    & Rotation error [deg]    & 75.3 & 67.3 & 15.9 & 1.48 & \textbf{1.12}     \\
                    & Translation error [m]  & 5.83 & 1.33 & 0.300 &  \textbf{0.0200} &  0.0499       \\
                    & IoU                & 0.755 & 0.398 & 0.729 & 0.825 & \textbf{0.970}      \\                                                               
\hline
\end{tabular}
}
\label{table:pascal3d}
\vspace{-6mm}
\end{table}

==> tex/table2.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
\caption{Results for synthetic PASCAL3D+ dataset. Experiment 1: Noiseless. Experiment 2: with additive Gaussian noise. Experiment 3: with additive Gaussian noise and 2 objects with the same motion.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l}
\hline
                    & Metric & \multicolumn{5}{c}{Method}    \\
\cline{3-7}
                    & (Median) & Naive & SRANSAC & T-Linkage         & Ours (Vanilla) & Ours \\
\hline
\hline
\multirow{4}{*}{1}  & Per-point Error [m]    &   0.787 & \textbf{0.0661} &  2.35 &  0.339 & 0.339    \\
                    & Rotation error [deg]     &   6.03e-7 & \textbf{0.0} & 5.96 & \textbf{0.0} & \textbf{0.0}    \\
                    & Translation error [m]  &   5.21e-14 & \textbf{3.44e-14} & 7.34e-14 & 3.55e-14 & \textbf{3.44e-14}    \\
                    & IoU                &   0.603 & \textbf{0.965} & 0.708 & 0.850 & 0.851     \\
\hline
\multirow{4}{*}{2}  & Per-point Error [m]   &   0.181 & 0.457 & 0.359 & 0.0758 &  \textbf{0.0548}     \\
                    & Rotation error [deg]    &   93.4 & 79.8 &  60.5 & 11.1 & \textbf{10.7}    \\
                    & Translation error [m]  &   1.03  & 0.853 & 0.658 & 0.117 & \textbf{0.116}   \\
                    & IoU                &    0.729 & 0.324 & 0.785 & 0.799 & \textbf{0.836}    \\ 
\hline
\multirow{4}{*}{3}  & Per-point Error [m]    & 0.124 & 0.538 & 0.929 &  0.0727 & \textbf{0.0297}   \\
                    & Rotation error [deg]    & 81.8 & 74.7 & 48.9 & 13.3 & \textbf{8.73}     \\
                    & Translation error [m]  & 5.014 & 0.88 & 2.50 &  0.170 &  \textbf{0.154}       \\
                    & IoU                & 0.747 & 0.296 & 0.767 & 0.698 & \textbf{0.874}      \\                                                               
\hline
\end{tabular}
}
\label{table:pascal3d}
\vspace{-6mm}
\end{table}

==> tex/theory-arxiv.tex <==
%!TEX root = ../main.tex

\section{Theoretical Analysis}
\label{sec:theory}

In this section, we theoretically show that \Cref{alg:EM} recovers the ground truth clusters 
under suitable condition on the initial clusters. In particular, we intend to keep all the constants and avoid using big O notation as constants matter when applying this algorithm to safety-critical applications in autonomous systems.

We say that a set of points $P$ is 
\emph{$\tau$-connected} if between any pair of points $\vxx, \vy \in P$ there is a sequence of points in $P$ such that every pair of consecutive points in the sequence are at most at distance $\tau$ from each other. 
Then, we say that a set of correspondences $S := \{(\va_i, \vb_i) \}_{i=1}^n$ is $\tau$-connected if $\{\va_i\}_{i=1}^n$ is $\tau$-connected.

To setup the problem formulation, we make the following assumptions. % ground truth. 
% The error of a hypothesis $h$ on a point cloud $S$ by $\err(h; S) := \E_{(\va, \vb) \sim S} [\norm{h(\va) - \vb}^2]$. 
% For us, $h(\va)$ will be of the form $\MR \va + \vt$ for some rotation $\MR$ and translation $\vt$. 

\begin{definition}[Problem Setup]\label{set:problem}
We are given a set of correspondences $S := \{(\va_i, \vb_i) \}_{i=1}^n$, 
which can be partitioned into $M$ $\tau$-connected parts $G_1, \dots, G_M$ such that
there are rigid transformations $(\MR_j, \vt_j), j \in [M]$ satisfying:
% there are functions $g_1, \dots, g_M$ of the form $g_j = \MR_j \va + \vt_j$ where $(\MR_j, \vt_j)$ is a rigid transformation, satisfying:
\begin{enumerate}
\item \textbf{Uniform Bounded Noise:} 
For all $j \in [M]$ and $(\va, \vb) \in G_j$, 
% $g_j(\va) + \vepsilon = \vb$, 
$ \MR_j \va + \vt_j  + \vepsilon = \vb$, 
where $\vepsilon$ is drawn from the {uniform} distribution over $ [-\sigma, \sigma]^3$. \label{item:GT}
\item \textbf{Object Separation:} 
For all distinct $i, j \in [M]$, 
$\min_{\va \in G_i, \va' \in G_j} \norm{\va - \va'} > \tau$. \label{item:ObjSep}
\item \textbf{Bounded Point Cloud:} 
For all $i \in [n]$, $\norm{\va_i}\leq B$. 

% \item \textbf{Signal separation:} For any sample $(\va, \vb)$, if $(\va, \vb) \notin G_i$ then $\norm{g(\va) - \vb} \geq \tau_S$.
\item \textbf{Outliers:} 
Some of the samples may be ``outliers''. 
We say that a point 
$(\va_o, \vb_o)$ is an outlier if, for all $j \in [M]$, ${d_{\text{cluster}}(G_j, (\va_o, \vb_o))> \tau}$. 
% For all distinct $i, j \in [k]$, 
% % $\norm{\MR_i - \MR_j} \geq \tau_{\MR}$.  } 
% \item \textbf{Non-degenerate objects:} Every $G_i$ is such that every $d+1$ points in $G_i$ are in general position.\label{item:NdO}
% \item \textbf{Good clustering:} \new{...} 
\end{enumerate}

\end{definition}

For \Cref{alg:EM} to converge, 
we will require good initial clustering. 
Here we formalize the definition of a good initial clustering: 
\begin{definition}[Good Clustering]\label{def:initial_conditions}
In the setting of Definition \ref{set:problem},
we say that the initial clustering 
$\cH := \{H_1, \dots, H_{K} \}$ with $K \geq M$ is $(\tau,\alpha, m_0)$-good, 
if it is a partition of the correspondences $S$ (as defined in Definition \ref{set:problem}) 
satisfying:
\begin{enumerate}
\item \textbf{$\tau$-connected:} 
For all $j \in [K]$,  $H_j$ is $\tau$-connected.
\label{item:tau-connected}
\item \textbf{Large Initial Clusters:} 
For all $j \in [K]$, $|H_j| \geq m_0$. \label{item:LargeObjects}
\item \textbf{Identifying cluster:} 
 For each ground truth cluster $G$, let $\cH_G := \{ H \in \cH \mid |H \cap G| > 0 \}$ and $H^* := \argmax_{H \in \cH_G} |H|$. Then, for some $\alpha > 1$, $|H^*| > \alpha \max_{H \in \cH_G \setminus \{H^*\} }|H|$.
% there is an $H \in \cH$ satisfying $|H \cap G| > 0$ such that 
% $|H| \geq \alpha \max \{ |H'| \mid |H' \cap G| > 0, H' \in \cH \setminus \{H\}  \}$. 
\label{item:identifying-cluster}
\end{enumerate}
\end{definition}

Intuitively, the last condition captures the idea that for any ground truth cluster $G$, the largest cluster having a nonzero intersection with $G$, namely $H^*$, is notably larger than all other initial clusters having a nonzero intersection with $G$. 

We first prove a lemma showing that for data subject to uniform zero-mean and bounded noise, Horn's method~\cite{Horn87josa, yao2023apla} results in a solution which can be made arbitrarily close to the true solution with a large enough number of samples. We define a simplified version of the Hoeffding's inequality specifically for analyzing our algorithm.
% initial cluster which intersects with ithere is one initial cluster 
% for each , 
% which is notably larger than all other clusters intersecting with the ground truth.
% which contains a relatively large fraction of the ground truth.
% More precisely,
% \begin{lemma}[Consistency]
% \label{lem:Horn}
% Let $\{ (\va_i, \vb_i) \}_{i=1}^m \subset \!\Real{3}\! \times\! \Real{3}$ be $m$ samples satisfying 
% $\vb_i = \MR \va_i + \vt + \vepsilon_i$ where $\vepsilon_i$ is drawn uniformly from $[-\sigma, \sigma]^3$, $\MR \in \SOthree$ is a rotation matrix and $\vt \in \Real{3}$ is a translation vector. Let $\Sigma \!=\! \frac 1 m \sum_i \va'_i (\va'_i)\tran$, where $\va_i' := \va_i - \frac 1 n \sum_{i=1}^n \va_i$.
% Then, with probability $1\!-\!2 \delta$, Horn's method returns $(\hat \MR, \hat \vt)$ such that 
% \begin{align*}
% \|\hat \MR - \MR\|_F^2 \leq \frac {18 B \sigma}{\lambda_{min}(\MSigma)}\sqrt{\frac{2}{m} \log \frac {18} \delta }
% \end{align*}
% and,
% \begin{align*}
% \| \hat \vt - \vt \|_2^2 \leq  36 B \sigma  \sqrt{\frac{2}{m} \log \frac {18} \delta } +
% \frac{12}{m} \sigma^2 \log \frac {6} \delta 
% \end{align*}
% \end{lemma}
% We then use Lemma~\ref{lem:Horn}  to demonstrate that our algorithm recovers the ground truth partitions, as shown below. 

% \begin{theorem}[Expectation-Maximization Guarantee]
% \label{thm:EM}
% In the setting of Definition \ref{set:problem}, 
% assume that the initial clustering $\cH$ is 
% $(\tau,\alpha,m_0)$-good in the sense of Definition \ref{def:initial_conditions}, where $m_0 \geq 2.5 \cdot 10^8  (\frac{\alpha+1}{\alpha-1})^2 \log \frac {18} {\delta} \max\left\{\frac{B^4}{\lambda^2},  B^2 , \sigma, 0.1 \right\}$ 
% % is some sufficiently large polynomial function of $1/\alpha, 1/\sigma_j$ and $\log(1/\delta)$, 
% where $\delta$ is the probability of failure of the algorithm and $\lambda$ is the smallest eigenvalue of {$\frac 1 m \sum_i \va'_i (\va'_i)\tran$.}
% Then, the partition $\cH'$ returned by \Cref{alg:EM} {recovers each of the ground truth clusters} (\eg the objects and background) with probability $1-\delta$.
% % returns $\cH'$, a partition of the set of correspondences $S$, {recovering each of the ground truth clusters} (\ie the objects and background). 
% \end{theorem}

% % We now sketch a proof outline of our main theoretical guarantee. 
% \emph{Intuition:}
% The proof of~\Cref{thm:EM} follows by noting that the initial clustering results in a partition of each ground truth cluster such that one of the set in the partition is notably larger than the rest. 
% As the algorithm progresses, the M-step assigns more points to the biggest estimated cluster until it  exactly matches the ground truth object which contains it. 
% This happens because the likelihood term $W_{i,j;\tau}$ in \Cref{alg:EM} is dominated by the weight term $\pi_j$ of the largest cluster. 

% \begin{remark}[Novelty]
% Similar to theoretical analyses of the EM algorithm in prior work in the context of learning a mixture of linear regressions, we require a good initialization, see,~\eg \cite{kwon20aistats-EM-MLR}. However, 
% contrary to related work, we do not assume the regressors (roughly speaking the vectors $\va_i$) to follow a Gaussian distribution, which would be too strict of an assumption in practical multi-modal registration problems. 
% % Moreover, we do not limit ourselves to linear regression.
% %and we solve a registration problem rather than linear regression.
% % As we will see in the next section, our assumptions in~\Cref{thm:EM} are fairly mild in practice.
% % these analyses are very specific to the case where the measurements are Gaussian and their initialization does not apply to real-world settings. 
% % We instead define a notion of good initialization which we can achieve using preexisting algorithms 
% % % to get an initial clustering of the given point cloud, 
% % and show that \Cref{alg:EM} converges given such an initialization.
% \end{remark}

==> tex/theory-icra.tex <==
%!TEX root = ../main.tex

\section{Theoretical Analysis}
\label{sec:theory}

In this section, we sketch a proof demonstrating that \Cref{alg:EM} recovers the ground truth clusters 
under suitable condition on the initial clusters.
In the following, we say that a set of points $P$ is 
\emph{$\tau$-connected} if between any pair of points $\vxx, \vy \in P$ there is a sequence of points in $P$ such that each pair of consecutive points in the sequence are at most at distance $\tau$ from each other. 
Then we say that a set of correspondences $S := \{(\va_i, \vb_i) \}_{i=1}^n$ is $\tau$-connected if $\{\va_i\}_{i=1}^n$ is $\tau$-connected.

We make the following assumptions on the ground truth. 
% The error of a hypothesis $h$ on a point cloud $S$ by $\err(h; S) := \E_{(\va, \vb) \sim S} [\norm{h(\va) - \vb}^2]$. 
% For us, $h(\va)$ will be of the form $\MR \va + \vt$ for some rotation $\MR$ and translation $\vt$. 

\begin{definition}[Ground Truth]\label{set:problem}
We are given a set of correspondences $S := \{(\va_i, \vb_i) \}_{i=1}^n$, 
which can be partitioned into $M$ $\tau$-connected parts $G_1, \dots, G_M$ such that
there are functions $g_1, \dots, g_M$ of the form $g_j = \MR_j \va + \vt_j$ where $(\MR_j, \vt_j)$ is a rigid transformation, satisfying:
\begin{enumerate}
\item \textbf{Uniform Bounded Noise:} 
For all $j \in [M]$ and $(\va, \vb) \in G_j$, 
$g_j(\va) + \vepsilon = \vb$, 
where $\vepsilon$ is drawn from the uniform distribution over $ [-\sigma, \sigma]^3$. \label{item:GT}
\item \textbf{Object Separation:} 
For all distinct $i, j \in [M]$, 
$\min_{(\va,\vb) \in G_i, (\va',\vb') \in G_j} \norm{\va - \va'} > \tau$. \label{item:ObjSep}
\item \textbf{Bounded Point Cloud:} 
For all $i \in [n]$, $\norm{\va_i}\leq B$. 

% \item \textbf{Signal separation:} For any sample $(\va, \vb)$, if $(\va, \vb) \notin G_i$ then $\norm{g(\va) - \vb} \geq \tau_S$.
\item \textbf{Outliers:} 
Some of the samples may be ``outliers''. 
We say that a point 
$(\va_o, \vb_o)$ is an outlier if, for all $j \in [M]$, $d_{\text{cluster}}(G_j, (\va_o, \vb_o))> \tau$. 
% For all distinct $i, j \in [k]$, 
% % $\norm{\MR_i - \MR_j} \geq \tau_{\MR}$.  } 
% \item \textbf{Non-degenerate objects:} Every $G_i$ is such that every $d+1$ points in $G_i$ are in general position.\label{item:NdO}
% \item \textbf{Good clustering:} \new{...} 
\end{enumerate}

\end{definition}

For \Cref{alg:EM} to converge, 
we will require good initial clustering (in Section~\ref{sec:experiments}, we show that using a simple Euclidean clustering 
or more modern alternatives, like SegmentAnything (SAM)~\cite{Kirillov23arxiv-SAM}, suffices). 
Here we formalize what it means to have good initial clustering: 
\begin{definition}[Good Clustering]\label{def:initial_conditions}
In the setting of Definition \ref{set:problem},
we say that the initial clustering 
$\cH := \{H_1, \dots, H_{K} \}$ with $K \geq M$ is $(\tau,\alpha, m_0)$-good, 
if it is a partition of the correspondences $S$ (as defined in Definition \ref{set:problem}) 
satisfying:
\begin{enumerate}
\item \textbf{$\tau$-connected:} 
For all $j \in [K]$,  $H_j$ is $\tau$-connected.
\label{item:tau-connected}
\item \textbf{Large Initial Clusters:} 
For all $j \in [K]$, $|H_j| \geq m_0$. \label{item:LargeObjects}
\item \textbf{Identifying cluster:} 
 For each ground truth cluster $G$, let $\cH_G := \{ H \in \cH \mid |H \cap G| > 0 \}$ and $H^* := \argmax_{H \in \cH_G} |H|$. Then, for some $\alpha > 1$, $|H^*| > \alpha \max_{H \in \cH_G \setminus \{H^*\} }|H|$.
% there is an $H \in \cH$ satisfying $|H \cap G| > 0$ such that 
% $|H| \geq \alpha \max \{ |H'| \mid |H' \cap G| > 0, H' \in \cH \setminus \{H\}  \}$. 
\label{item:identifying-cluster}
\end{enumerate}
\end{definition}

Intuitively, the last condition captures the idea that for any ground truth cluster $G$, the largest cluster having a nonzero intersection with $G$, namely $H^*$, is notably larger than all other initial clusters having a nonzero intersection with $G$. 
% initial cluster which intersects with ithere is one initial cluster 
% for each , 
% which is notably larger than all other clusters intersecting with the ground truth.
% which contains a relatively large fraction of the ground truth.
% More precisely,

\begin{theorem}[Expectation-Maximization Guarantee]
\label{thm:EM}
In the setting of Definition \ref{set:problem}, 
assume that the initial clustering $\cH$ is 
$(\tau,\alpha,m_0)$-good in the sense of Definition \ref{def:initial_conditions}, for some sufficiently large $m_0$.
% some sufficiently large polynomial function of $1/\alpha, 1/\sigma$ and $\log(1/\delta)$, where $\delta$ is the probability of failure of the algorithm.
Then, running \Cref{alg:EM}, with high probability (dependent on $m_0$),
returns $\cH'$, a partition of the set of correspondences $S$, {containing each of the ground truth clusters} (\ie the objects and background). 
% $\cH'$  such that for every $h' \in \cH'$ satisfies,
% $\min_{G_i \in \cG} \err(h';G_i) \leq \eps$.  
\end{theorem}

% We now sketch a proof outline of our main theoretical guarantee. 
\emph{Intuition:}
The proof of~\cref{thm:EM} follows by noting that the initial clustering results in a partition of each ground truth cluster such that one of the partitions is notably larger than the rest. 
As the algorithm progresses, the M-step assigns more points to the biggest estimated cluster until it exactly matches the ground truth object which contains it. 
This happens because the likelihood $W_{i,j;\tau}$ is maximized by the largest cluster, due to the 
presence of the weight $\pi_j$ (\ie the cluster size).
% dominated by the weight term $\pi_j$ of the largest cluster. 

\emph{Proof Sketch:}
We make the following observations, which together imply that the final clusters produced by~\Cref{thm:EM}  include the ground truth clusters. 
First, {each ground truth-cluster is partitioned by the initial clustering}. This is because
% one element of which is $\alpha$-times larger than all the others.
the $\tau$-connected subsets of the data either consist of samples that are entirely contained in one of the $G_j$ or (possibly) the set of outliers. Since the initial clustering $\cH$ exclusively consists of $\tau$-connected subsets, % and is a partition of $S$, 
each element of $\cH$ is either a subset of $G_j$ for some $j$ or entirely consists of outliers.

Now %now set up some convention for what follows.
suppose the weights for the clusters are given by $\pi_1, \dots, \pi_{K}$.
Without loss of generality, suppose $\{ H_1, \dots, H_t \}$ form a partition of $G_1$ 
with $\pi_1 \geq \dots \geq \pi_{t}$. Since $\cH$ is $(\tau,\alpha, m_0)$-good,
we know that $\pi_1 > \alpha \pi_2$ because of \Cref{item:identifying-cluster} in Definition~\ref{def:initial_conditions}. 
Our second claim is that in each iteration of the $M$-step,
elements of $S$ that are $\tau$-close to the largest cluster $H_1$ are assigned to $H_1$. 
To see this, consider a point $(\va_i, \vb_i) \in G_1 \setminus H_1$ which is $\tau$-close to $H_{1}$ (if no such point exists, then $H_1 = G_1$). We show that for the point $(\va_i, \vb_i)$, the likelihood term $W_{i,j;\tau}$ is maximized when $j=1$. 
% This will follow from the fact that $W_{i,1;\tau}$ is much larger than $W_{i,j;\tau}$ for all $j\in[t] \setminus \{1\}$ because $\pi_1$ is much larger than the weights for the other clusters.


Since Horn's Method is consistent (\ie for a sufficiently large sample size, the algorithm converges to the true solution in the presence of zero-mean  noise) and the domain of the point-cloud is bounded by a ball of radius $B$, $h_j := \MR_j^{(r)}\va_i + \vt_j^{(r)}$ and $\sigma_j$ estimate $g_1$ and $\sigma$ up to an additive error of $\eps'$, according to standard concentration results. 
Choosing sufficiently large $m_{\min}$ and $m_0$ ensures that the sample size is large and consequently that $\eps'$ is small.
% \red{A large sample size can be ensured by letting $m_{\min}$ and $m_0$ be a sufficiently large polynomial function of $1/\eps', 1/\sigma$, and $\log(1/\delta)$, where $\delta$ is the probability of success.} 
% Then, for all $H_j$ such that $|H_j|$ is large enough, our estimates $h_j$ and $\sigma_j$ converge to the corresponding ground truth parameters ($g_1$ and $\sigma$). 
This is enforced by the algorithm, which deletes candidate clusters of size less than $m_{\min}$.
% Moreover, note that any cluster that is smaller than $m_{\min}$  is deleted by the algorith
 % if $|H_j|$ is much smaller than $m_\min$, then we delete the cluster $H_j$ from our set of candidate clusters. 
Now note that $\argmax_j W_{i,j;\tau} 
 = \argmax_j \pi_j \phi_j(\vb_i \mid \va_i) 
 = \argmax_j \pi_j \exp(-\norm{\vb_i - h_j(\va_i) }^2/{\sigma_j}^2) {/\sigma_j}$. 
Since $\eps'$ is sufficiently small for large sample size, we get
$W_{i,j;\tau}= \pi_j (1\pm \eps) \exp(-\norm{\vb_i - g_1(\va_i)}^2/{\sigma}^2)/\sigma$, where $\eps$ is a function of $\eps', \sigma$, and $B$.
 % we see that for a sufficiently large $H_j$ for $j \in [t]$, 
 % $h_j$ converges to $g_1$ on the domain of the point-cloud, 
 % i.e. $|h_j(\va_i) - g_1(\va_i)| \leq \eps'$. 
%
% Similarly, it can be shown that our estimate of the standard deviation of the noise is also correct upto an additive error of $\eps'$.
% true for our estimate of the standard deviation of the noise.
%
% Let $\sigma$ denote the standard deviation of the noise in $G_1$ with respect to the ground truth rotation and translation $g_1$. 
%
% (the bound on the norm of the elements of the point cloud). 
Since $\exp(-\norm{\vb_i - g_1(\va_i)}^2/{\sigma}^2)/\sigma$ is a constant with respect to $j$, it does not affect the maximization. 
This implies 
% $\argmax_j W_{i,j;\tau}=\argmax_j \pi_j (1\pm 3\eps)$, and so 
$\argmax_j W_{i,j;\tau}$ is essentially determined by $\argmax_j \pi_j (1\pm \eps)$. Choosing small $\eps$ to ensure $(1+\eps)/(1-\eps) < \alpha$ and recalling that $\pi_1 > \alpha \pi_2$, we see $\argmax_j W_{i,j;\tau} = \argmax_j \pi_j (1\pm \eps) = 1$. Since $\pi_1$ keeps increasing in size at each iteration, eventually all the elements of $G_1$ will collect into $H_1$. 
\qed
% To see this, observe that since each $H_i$ is sufficiently large, 
% with high probability,
% Horn's method will converge to the true rotation $g_1$,
% and our estimate of the standard deviation of the noise in each of the partitions will be close to the standard deviation of the noise with respect to $g_1$ for the samples in $G_1$.
% A short calculation then demonstrates that $\argmax_j W_{i,j;\tau}$ is essentially determined by $\argmax_j \pi_j (1\pm 3\eps)$ when $\eps$ is small enough. Choosing $\eps$ to ensure $(1+\eps)/(1-\eps) < \alpha$ and recalling that $\pi_1 > \alpha \pi_2$, we see $\argmax_j W_{i,j;\tau} = \argmax_j \pi_j (1\pm \eps) = 1$. Since $\pi_1$ keeps increasing in size in each iteration, eventually all the elements of $G_1$ will collect into $H_1$. 

% Since each $H_i$ is sufficiently large, with high probability,
% Horn's method will converge to the true rotation $g_1$,
% and our estimate of the standard deviation of the noise in each of the partitions will be close to the standard deviation of the noise with respect to $g_1$ for the samples in $G_1$.

% \red{
% satisfying certain conditions (which we observe in our experiments),
% namely, (i) $\cH$ is a partition of $S$;
% (ii) Every ground truth cluster contains at least one cluster from $\cH$ that is relatively large compared to the others; and
% (iii) Every cluster in the initial clustering is not too small, and is $\tau$-connected.
% \myparagraph{Preliminaries and Notation}
% We provide the following notation and definitions that we will use in this and the following section. 

\begin{remark}[Novelty]
Similar to theoretical analyses of the EM algorithm in prior work in the context of learning a mixture of linear regressions, we require a good initialization, see,~\eg \cite{kwon20aistats-EM-MLR}. However, 
contrary to related work, we do not assume the regressors (roughly speaking, the vectors $\va_i$) to follow a Gaussian distribution, which would be too strict of an assumption in practical multi-modal registration problems. 
% Moreover, we do not limit ourselves to linear regression.
%and we solve a registration problem rather than linear regression.
% As we will see in the next section, our assumptions in~\Cref{thm:EM} are fairly mild in practice.
% these analyses are very specific to the case where the measurements are Gaussian and their initialization does not apply to real-world settings. 
% We instead define a notion of good initialization which we can achieve using preexisting algorithms 
% % to get an initial clustering of the given point cloud, 
% and show that \Cref{alg:EM} converges given such an initialization.
\end{remark}
% \blue{Sushrut: Removed even more calculation, hopefully this is okay.}
% $\exp(-\norm{g_1(\va_i) - \vb_i}^2/{{\sigma^*}_1}^2)/{\sigma^*}_1$ for $\eps$ chosen to be sufficiently small. Since the second term is a constant with respect to $j$, by choosing $\eps$ to be sufficiently small we can ensure $(1+\eps)/(1-\eps) < \alpha$, and so $\argmax_j W_{i,j;\tau} = \argmax_j \pi_j (1\pm \eps) = 1$. 
% (i.e. smaller than $(1-\alpha)(1/3)$)
% $\argmax_j W_{i,j;\tau} 
% = \argmax_j \pi_j \phi_j(\vb_i \mid \va_i) 
% = \argmax_j \pi_j \exp(-\norm{h_j(\va_i) - \vb_i}^2/{\sigma_j}^2)/\sigma_j 
% = \argmax_j \pi_j (1\pm \eps') \exp(-\norm{g_1(\va_i) - \vb_i}^2/{{\sigma^*}_1}^2)/{\sigma^*}_1 
% = 1$. 
% The second-to-last equality is a consequence of choosing $\eps$ sufficiently small,
% and $\eps'$ satisfying $1+\eps' < \alpha$. 


% The final equality follows from the facts that (i) the partitions are independent of the noise
% (ii) both Horn's method and the empircal estimate of the standard deviation are consistent, 
% and converge to the true mean.

% It is easy to see that if $\pi^{(r)}_q < (1-3\eps)\pi^{(r)}_{i^*}$, 
% then then all the samples in $H_q$ will be reassigned to $H_{i^*}$.

% \emph{Noiseless setting:}



% \emph{With Noise:}

% Our proof proceeds in $2$ steps:

% First, the initial clustering $\cH := \{ H_1, \dots, H_{M} \}$ is such that each of the $H_i$ is either a subset of $G_j$ for some $j$ or entirely consists of outliers.
% This is because the only $\tau$-connected subsets of the data either consist of samples that are entirely contained in one of the $G_i$ or (possibly) the set of outliers. 
% Second, In each iteration, the mass on the ground truth clusters concentrates. 

% To see this, suppose that during the $r^{th}$ iteration,
% the weights for the $M$ hypotheses are given by $\pi^{(r)}_1, \dots, \pi^{(r)}_{M}$.
% Let $i^* := \argmax_i \pi_i^{(r)}$. 
% Of these, suppose without loss of generality that for some $t \geq 1$, 
% hypotheses $H_1, \dots, H_t \subset G_1$,
% and $\cup_{i=1}^t H_i = G_1$. 
% Then, 
% \begin{enumerate}
%     \item If $\pi^{(r)}_{i^*}$ is sufficiently large (larger than $(1+3\eps)$ times the second largest in the set $\{ \pi_i^{(r)} \}_{i=1}^{M}$), then in the M-step, every sample that is $\tau$-close to  $H_{i^*}$ gets assigned to $i^*$. \label{item:large_sufficient}
%     \item Since each of the ground-truth sets are $\tau$-connected, there are always samples close to the largest cluster which will keep getting accumulated. 
%     \item Since the noise $\eps$ is much smaller than $\tau$, we see that the variance cannot 
% \end{enumerate}
%     To see \Cref{item:large_sufficient}, observe that 
%     This is because for any $(\va_i, \vb_i)$ which is $\tau$-close to $H_{i^*}$, 
%     $\argmax_j W^{(r)}_{i,j;\tau} 
%     = \argmax_j \pi^{(r)}_j \phi^{(r)}_j(\vb_i \mid \va_i) 
%     = \argmax_j \pi^{(r)}_j \exp(\norm{h_j(\va_i) - \vb_i}^2/{\sigma^{(r)}_j}^2)/\sigma^{(r)}_j = \argmax_j \pi^{(r)}_j (1\pm \eps) \exp(\norm{g_1(\va_i) - \vb_i}^2/{{\sigma^*}_1}^2)/{\sigma^*}_1 
%     = i^*$. 
%     The final equality follows from the fact that 
%     each of the $h_j$ are 


% Then, it is easy to see that if some point $(\va_i, \vb_i) \in H_1$, 
% line $18$ of the algorithm will assign the point $p_j$ to the hypothesis indexed by $f(i) := \argmax_j W_{i,j;\tau}^{(r)}$. 
% The convention the algorithm uses is that $f(i)$ will be the smallest index
% among all the possible candidates which achieve the largest value. 
% We will show that if $\pi^{(r)}_1$ is sufficiently large,
% then all the mass gets concentrated in $H_1$.
% If this is not the case, then $\pi^{(r)}_1$ will eventually
% become sufficiently large. 
% To see the first claim, we make the following observations: 
% (i) Since each $H_i$ is sufficiently large, and independent of the noise. The sample variance of each of the sets $H_1, \dots, H_t$, $\sigma^{(r)}_{i} = \sigma_1 (1 \pm \epsilon)$. 
% (ii) If $\pi^{(r)}_1 \geq (1+\eps) \pi^{(r)}_{2}$, then every sample in $H_1 \cup \dots \cup H_t$ goes to $H_1$. 


% $
% = \argmax_j  \frac{ \pi_j^{(r)}\phi_k^{(r)}(\vb_i | \va_i)}{\sum_{j=1}^g \pi_j^{(r)} \phi_j^{(r)}(\vb_i | \va_i) } 
% \cdot \mathbf{1}(d_{\text{cluster}}(H_j, (\va_i, \vb_i)) < \tau)$.
% This is nonzero only if the distance from $H_j$ to  $(\va_i, \vb_i)$ is at most $\tau$.
% This ensures that the point $(\va_i, \vb_i)\in G_1$ 
% cannot be assigned to any $G_j$ where $j \neq 1$. 
% If the value is indeed nonzero, then in the next iteration $r+1$, 
% the point $(\va_i, \vb_i)$ will be assigned to the hypothesis $H_j$
% where $j = \argmax_{j \in [t]} \pi_j^{(r)}\phi(0,{\sigma^{(r)}}_j^2)$.
% We put the hypothesis in the smallest index cluster if all entries are the same.
% However, since with probability 
% \snote{1. show big clusters get bigger. 
% 2. If equal sized cluster then the preference is to a lower index.}

% Since $|H_i| \geq \Omega(\frac{1}{\eps^2} \log(1/\delta))$ we know that Horn's Method recovers a hypothesis $h_i$ that is close to $g_j$ (see \cite{}). 
% \snote{don't talk about $h_i$, these will keep getting updated later. $H_i$ depends on the original noise gaussian}

% \hide{\new{
% We will show that given a good initialization,
% it is possible to recover the right hypotheses.
% To this end, we demonstrate the following.

% \emph{1. The ``good hypotheses" are never eliminated:}
% To see this, observe that the error a point $\vp$ makes with respect to the target hypothesis is small.
% This is because the rotations are well-separated. 
% Additionally, note that the likelihood of such a point is going to be nonzero.


% \emph{2. Any hypothesis that makes an error of more than $10\tau$ with the original hypothesis is eliminated.}
% To see this, suppose to the contrary that there is an h which is far from all the $g_1, .., g_|G|$.but makes an error of $\leq \tau$ for each of these.This means there is at least one $G_i$ which overlaps with $h$ significantly.
% But this means $h(x) - y = g(x) - y \pm \tau$ and so $h(x) - g(x) = O(\tau)$.
% but this in turn means that $h$ and $g$ are close.so the number of points that $h$ explains has to be smaller than \new{???}.If so, it gets eliminated..

% \emph{3. Among the good hypotheses the points that correspond to that object eventually collect}
% Let the ground truth be let $p \in G_i$ and suppose the samples are


% \snote{Need to first find weights, then cluster together etc. This will help collect things. Which will eventually converge. }

% }
% We will discuss this in the noiseless setting first.

% \paragraph{Noiseless}

% We know from the setting of the problem (\Cref{set:problem})
% that $|G_i| \geq \gamma |S|$. 

% Let $\cH_{\geq}$ denote the subset of $\cH$ such that for every $h \in \cH_{\geq}$,
% $|H_0(h)| \geq \gamma |S|$, where 
% $H_\eta(h) := \{ (x, y) \in S \mid \err(h; \{(x, y)\}) \leq \eta \}$. 
% Now, since $S$ is partitioned into $G_1, \dots, G_k$, 
% it must be the case that each $H_0(h)$ has some overlap with some of the $G_i$. 
% Since the setting is non-degenerate (\Cref{item:NdO} from \Cref{set:problem}), 
% If $|H_0(h) \cap G_i| \geq (d+1)$ where $d$ is the dimension (in our case a constant),
% then $h \equiv g_i$. 
% Otherwise $|H_0(h)| \leq (d+1) k$. 
% However, since $m > (d+1) k/\gamma$, and $|H_0(h)| \geq \gamma |S|$,
% we see that $h \notin \cH'$.
% Hence every $h \in \cH'$ is a ground truth hypothesis.
% Also, no ground truth hypothesis is removed, since $G_i \subset H_0(g_i)$ for every $i \in [k]$. \snote{$\cH'$ and $\cH_{\geq}$. Make them the same.}

% \paragraph{Randomly Selected Arbitrary Outliers}

% Suppose an $\eps$ fraction of the samples $S$ are corrupted arbitrarily,
% but the location of these corruptions is uniform at random
% (this ensures that no object gets completely hidden).

% In the absence of any other noise, the previous argument still goes through.
% \snote{Okay, but how will you ensure good initial estimates via clustering?
% I think the right clustering strategy will not cluster the outliers with the inliers
% unless they are close to being inliers, in which case it does not matter.}
% Let $I$ denote the set of inliers, and $O$ the set of outliers, and $I \cup O = S$.
% If a hypothesis $h$ satisfies 
% $|H_0(h) \cap H_0(g)| \geq \Omega((d+1)/(1-\eps) \log(1/\delta))$ for some $g \in \cG$, 
% then, with probability $1-\delta$, $|H_0(h) \cap H_0(g) \cap I| \geq \Omega(d+1)$. 
% in which case, $h \equiv g$. 
% If there is no $g$ for which $|H_0(h) \cap H_0(g)| \geq \Omega((d+1)/(1-\eps) \log(1/\delta))$,
% then it must be that $|H_0(h)| \leq O((k (d+1) / (1-\eps)) \log(1/\delta))$.
% As long as $|S|$ is large enough, once again, 
% we have a contradiction and $h$ should have been removed.
% \snote{also consider adversarial noise}

% \new{\paragraph{Bounded Additive Noise}

% Suppose each $g_i$ satisfies $\err(g_i; G_i) \leq \eta$. 
% We know from the setting of the problem (\Cref{set:problem}) 
% that $|G_i| \geq \gamma |S|$. 
% Let $\cH_{\geq}$ denote the subset of $\cH$ such that for every $h \in \cH_{\geq}$,
% $|H_\eta(h)| \geq \gamma |S|$.

% Now, since $S$ is partitioned into $G_1, \dots, G_k$, 
% it must be the case that each $H_\eta(h)$ has some overlap with some of the $G_i$. 

% Since the setting is non-degenerate (\Cref{item:NdO} from \Cref{set:problem}), 
% \new{If $|H_\eta(h) \cap G_i| \geq \gamma' |S|$ then $\err(h, G_i) \leq (\gamma/\gamma')$.} 
% Otherwise $|H_\eta(h)| \leq \gamma' k |S|$. 
% However, since $m > |S|/k\gamma'$, and $|H_\eta(h)| \geq \gamma |S|$,
% we see that $h \notin \cH'$.
% Hence every $h \in \cH'$ is a ground truth hypothesis.

% Also, no ground truth hypothesis is removed, 
% since $G_i \subset H_\eta(g_i)$ for every $i \in [k]$. 
% Suppose each for every $g \in \cG$ we have $|H_\eta(h) \cap H_\eta(g)| \leq \alpha |S|$
% and so $|H_\eta(h)| \leq k \alpha |S|$. }
% }

% \end{proof}

==> tex/theory-old.tex <==
%!TEX root = ../main.tex

\section{Theoretical Analysis}
\label{sec:theory}

In this section, we sketch a proof demonstrating that \Cref{alg:EM} recovers the ground truth clusters 
under suitable condition on the initial clusters.
In the following, we say that a set of points $P$ is 
\emph{$\tau$-connected} if between any pair of points $\vxx, \vy \in P$ there is a sequence of points in $P$ such that each pair of consecutive points in the sequence are at most at distance $\tau$ from each other. 
Then we say that a set of correspondences $S := \{(\va_i, \vb_i) \}_{i=1}^n$ is $\tau$-connected if $\{\va_i\}_{i=1}^n$ is $\tau$-connected.

We make the following assumptions on the ground truth. 
% The error of a hypothesis $h$ on a point cloud $S$ by $\err(h; S) := \E_{(\va, \vb) \sim S} [\norm{h(\va) - \vb}^2]$. 
% For us, $h(\va)$ will be of the form $\MR \va + \vt$ for some rotation $\MR$ and translation $\vt$. 

\begin{definition}[Ground Truth]\label{set:problem}
We are given a set of correspondences $S := \{(\va_i, \vb_i) \}_{i=1}^n$, 
which can be partitioned into $M$ $\tau$-connected parts $G_1, \dots, G_M$ such that
there are functions $g_1, \dots, g_M$ of the form $g_j = \MR_j \va + \vt_j$ where $(\MR_j, \vt_j)$ is a rigid transformation, satisfying:
\begin{enumerate}
\item \textbf{Uniform Bounded Noise:} 
For all $j \in [M]$ and $(\va, \vb) \in G_j$, 
$g_j(\va) + \vepsilon = \vb$, 
where $\vepsilon$ is drawn from the uniform distribution over $ [-\sigma, \sigma]^3$. \label{item:GT}
\item \textbf{Object Separation:} 
For all distinct $i, j \in [M]$, 
$\min_{\va \in G_i, \va' \in G_j} \norm{\va - \va'} > \tau$. \label{item:ObjSep}
\item \textbf{Bounded Point Cloud:} 
For all $i \in [n]$, $\norm{\va_i}\leq B$. 

% \item \textbf{Signal separation:} For any sample $(\va, \vb)$, if $(\va, \vb) \notin G_i$ then $\norm{g(\va) - \vb} \geq \tau_S$.
\item \textbf{Outliers:} 
Some of the samples may be ``outliers''. 
We say that a point 
$(\va_o, \vb_o)$ is an outlier if, for all $j \in [M]$, $d_{\text{cluster}}(G_j, (\va_o, \vb_o))> \tau$. 
% For all distinct $i, j \in [k]$, 
% % $\norm{\MR_i - \MR_j} \geq \tau_{\MR}$.  } 
% \item \textbf{Non-degenerate objects:} Every $G_i$ is such that every $d+1$ points in $G_i$ are in general position.\label{item:NdO}
% \item \textbf{Good clustering:} \new{...} 
\end{enumerate}

\end{definition}

For \Cref{alg:EM} to converge, 
we will require good initial clustering (in Section~\ref{sec:experiments}, we show that using a simple Euclidean clustering 
or more modern alternatives, like SegmentAnything (SAM)~\cite{Kirillov23arxiv-SAM}, suffices). 
Here we formalize what it means to have good initial clustering: 
\begin{definition}[Good Clustering]\label{def:initial_conditions}
In the setting of Definition \ref{set:problem},
we say that the initial clustering 
$\cH := \{H_1, \dots, H_{K} \}$ with $K \geq M$ is $(\tau,\alpha, m_0)$-good, 
if it is a partition of the correspondences $S$ (as defined in Definition \ref{set:problem}) 
satisfying:
\begin{enumerate}
\item \textbf{$\tau$-connected:} 
For all $j \in [K]$,  $H_j$ is $\tau$-connected.
\label{item:tau-connected}
\item \textbf{Large Initial Clusters:} 
For all $j \in [K]$, $|H_j| \geq m_0$. \label{item:LargeObjects}
\item \textbf{Identifying cluster:} 
 For each ground truth cluster $G$, let $\cH_G := \{ H \in \cH \mid |H \cap G| > 0 \}$ and $H^* := \argmax_{H \in \cH_G} |H|$. Then, for some $\alpha > 1$, $|H^*| > \alpha \max_{H \in \cH_G \setminus \{H^*\} }|H|$.
% there is an $H \in \cH$ satisfying $|H \cap G| > 0$ such that 
% $|H| \geq \alpha \max \{ |H'| \mid |H' \cap G| > 0, H' \in \cH \setminus \{H\}  \}$. 
\label{item:identifying-cluster}
\end{enumerate}
\end{definition}

Intuitively, the last condition captures the idea that for any ground truth cluster $G$, the largest cluster having a nonzero intersection with $G$, namely $H^*$, is notably larger than all other initial clusters having a nonzero intersection with $G$. 
% initial cluster which intersects with ithere is one initial cluster 
% for each , 
% which is notably larger than all other clusters intersecting with the ground truth.
% which contains a relatively large fraction of the ground truth.
% More precisely,

\begin{theorem}[Expectation-Maximization Guarantee]
\label{thm:EM}
In the setting of Definition \ref{set:problem}, 
assume that the initial clustering $\cH$ is 
$(\tau,\alpha,m_0)$-good in the sense of Definition \ref{def:initial_conditions}, where $m_0$ is some sufficiently large polynomial function of $1/\alpha, 1/\sigma$ and $\log(1/\delta)$, where $\delta$ is the probability of failure of the algorithm.
Then, running \Cref{alg:EM}, with probability $1-\delta$,
returns $\cH'$, a partition of the set of correspondences $S$, {containing each of the ground truth clusters} (\ie the objects and background). 
% $\cH'$  such that for every $h' \in \cH'$ satisfies,
% $\min_{G_i \in \cG} \err(h';G_i) \leq \eps$.  
\end{theorem}

% We now sketch a proof outline of our main theoretical guarantee. 
\emph{Intuition:}
The proof of~\cref{thm:EM} follows by noting that the initial clustering results in a partition of each ground truth cluster such that one of the partitions is notably larger than the rest. 
As the algorithm progresses, the M-step assigns more points to the biggest estimated cluster until it is exactly matches to the ground truth object which contains it. 
This happens because the likelihood term $W_{i,j;\tau}$ is dominated by the weight term $\pi_j$ of the largest cluster. 

\emph{Proof Sketch:}
We make the following observations, which together imply that the final clusters produced by~\Cref{thm:EM}  contain the ground truth clusters. 
First, {each ground truth-cluster is partitioned by the initial clustering}. This is because
% one element of which is $\alpha$-times larger than all the others.
the $\tau$-connected subsets of the data either consist of samples that are entirely contained in one of the $G_j$ or (possibly) the set of outliers. Since the initial clustering $\cH$ exclusively consists of $\tau$-connected subsets, % and is a partition of $S$, 
each element of $\cH$ is either a subset of $G_j$ for some $j$ or entirely consists of outliers.

Now %now set up some convention for what follows.
suppose the weights for the clusters are given by $\pi_1, \dots, \pi_{K}$.
Without loss of generality, suppose $\{ H_1, \dots, H_t \}$ form a partition of $G_1$ 
with $\pi_1 \geq \dots \geq \pi_{t}$. Since $\cH$ is $(\tau,\alpha, m_0)$-good,
we know that $\pi_1 > \alpha \pi_2$ because of \Cref{item:identifying-cluster} in Definition~\ref{def:initial_conditions}. 
Our second claim is that in each iteration of the $M$-step,
elements of $S$ that are $\tau$-close to the largest cluster $H_1$ are assigned to $H_1$. 
To see this, consider a point $(\va_i, \vb_i) \in G_1 \setminus H_1$ which is $\tau$-close to $H_{1}$ (if no such point exists, then $H_1 = G_1$). We show that for the point $(\va_i, \vb_i)$, the likelihood term $W_{i,j;\tau}$ is maximized when $j=1$. 
% This will follow from the fact that $W_{i,1;\tau}$ is much larger than $W_{i,j;\tau}$ for all $j\in[t] \setminus \{1\}$ because $\pi_1$ is much larger than the weights for the other clusters.


Since Horn's Method is consistent (to be consistent means that with a sufficiently large sample size, the algorithm converges to the true solution in the presence of zero-mean  noise) and the domain of the point-cloud is bounded by a ball of radius $B$, $h_j := \MR_j^{(r)}\va_i + \vt_j^{(r)}$ and $\sigma_j$ estimate $g_1$ and $\sigma$ up to an additive error of $\eps'$. 
\red{A large sample size can be ensured by letting $m_{\min}$ and $m_0$ be a sufficiently large polynomial function of $1/\eps', 1/\sigma$, and $\log(1/\delta)$, where $\delta$ is the probability of success.} 
% Then, for all $H_j$ such that $|H_j|$ is large enough, our estimates $h_j$ and $\sigma_j$ converge to the corresponding ground truth parameters ($g_1$ and $\sigma$). 
However, if $|H_j|$ is much smaller than $m_\min$, then we delete the cluster $H_j$ from our set of candidate clusters. 

Notice that $\argmax_j W_{i,j;\tau} 
 = \argmax_j \pi_j \phi_j(\vb_i \mid \va_i) 
 = \argmax_j \pi_j \exp(-\norm{\vb_i - h_j(\va_i) }^2/{\sigma_j}^2) \red{/\sigma_j}$. 
Choosing $\eps'$ to be sufficiently small, we get,
$\argmax_j W_{i,j;\tau}= \argmax_j \pi_j (1\pm \eps) \exp(-\norm{\vb_i - g_1(\va_i)}^2/{\sigma}^2)/\sigma$, where $\eps$ is a function of $\eps', \sigma$, and $B$.
 % we see that for a sufficiently large $H_j$ for $j \in [t]$, 
 % $h_j$ converges to $g_1$ on the domain of the point-cloud, 
 % i.e. $|h_j(\va_i) - g_1(\va_i)| \leq \eps'$. 

% Similarly, it can be shown that our estimate of the standard deviation of the noise is also correct upto an additive error of $\eps'$.
% true for our estimate of the standard deviation of the noise.

% Let $\sigma$ denote the standard deviation of the noise in $G_1$ with respect to the ground truth rotation and translation $g_1$. 
 
% (the bound on the norm of the elements of the point cloud). 

Since $\exp(-\norm{\vb_i - g_1(\va_i)}^2/{\sigma}^2)/\sigma$ is a constant with respect to $j$, it does not affect the maximization. 
This implies 
% $\argmax_j W_{i,j;\tau}=\argmax_j \pi_j (1\pm 3\eps)$, and so 
$\argmax_j W_{i,j;\tau}$ is essentially determined by $\argmax_j \pi_j (1\pm \eps)$. Choosing small $\eps$ to ensure $(1+\eps)/(1-\eps) < \alpha$ and recalling that $\pi_1 > \alpha \pi_2$, we see $\argmax_j W_{i,j;\tau} = \argmax_j \pi_j (1\pm \eps) = 1$. Since $\pi_1$ keeps increasing in size in each iteration, eventually all the elements of $G_1$ will collect into $H_1$. 
\qed
% To see this, observe that since each $H_i$ is sufficiently large, 
% with high probability,
% Horn's method will converge to the true rotation $g_1$,
% and our estimate of the standard deviation of the noise in each of the partitions will be close to the standard deviation of the noise with respect to $g_1$ for the samples in $G_1$.
% A short calculation then demonstrates that $\argmax_j W_{i,j;\tau}$ is essentially determined by $\argmax_j \pi_j (1\pm 3\eps)$ when $\eps$ is small enough. Choosing $\eps$ to ensure $(1+\eps)/(1-\eps) < \alpha$ and recalling that $\pi_1 > \alpha \pi_2$, we see $\argmax_j W_{i,j;\tau} = \argmax_j \pi_j (1\pm \eps) = 1$. Since $\pi_1$ keeps increasing in size in each iteration, eventually all the elements of $G_1$ will collect into $H_1$. 

% Since each $H_i$ is sufficiently large, with high probability,
% Horn's method will converge to the true rotation $g_1$,
% and our estimate of the standard deviation of the noise in each of the partitions will be close to the standard deviation of the noise with respect to $g_1$ for the samples in $G_1$.

% \red{
% satisfying certain conditions (which we observe in our experiments),
% namely, (i) $\cH$ is a partition of $S$;
% (ii) Every ground truth cluster contains at least one cluster from $\cH$ that is relatively large compared to the others; and
% (iii) Every cluster in the initial clustering is not too small, and is $\tau$-connected.
% \myparagraph{Preliminaries and Notation}
% We provide the following notation and definitions that we will use in this and the following section. 

\begin{remark}[Novelty]
Similar to theoretical analyses of the EM algorithm in prior work in the context of learning a mixture of linear regressions, we require a good initialization, see,~\eg \cite{kwon20aistats-EM-MLR}. However, 
contrary to related work, we do not assume the regressors (roughly speaking the vectors $\va_i$) to follow a Gaussian distribution, which would be too strict of an assumption in practical multi-modal registration problems. 
% Moreover, we do not limit ourselves to linear regression.
%and we solve a registration problem rather than linear regression.
% As we will see in the next section, our assumptions in~\Cref{thm:EM} are fairly mild in practice.
% these analyses are very specific to the case where the measurements are Gaussian and their initialization does not apply to real-world settings. 
% We instead define a notion of good initialization which we can achieve using preexisting algorithms 
% % to get an initial clustering of the given point cloud, 
% and show that \Cref{alg:EM} converges given such an initialization.
\end{remark}
% \blue{Sushrut: Removed even more calculation, hopefully this is okay.}
% $\exp(-\norm{g_1(\va_i) - \vb_i}^2/{{\sigma^*}_1}^2)/{\sigma^*}_1$ for $\eps$ chosen to be sufficiently small. Since the second term is a constant with respect to $j$, by choosing $\eps$ to be sufficiently small we can ensure $(1+\eps)/(1-\eps) < \alpha$, and so $\argmax_j W_{i,j;\tau} = \argmax_j \pi_j (1\pm \eps) = 1$. 
% (i.e. smaller than $(1-\alpha)(1/3)$)
% $\argmax_j W_{i,j;\tau} 
% = \argmax_j \pi_j \phi_j(\vb_i \mid \va_i) 
% = \argmax_j \pi_j \exp(-\norm{h_j(\va_i) - \vb_i}^2/{\sigma_j}^2)/\sigma_j 
% = \argmax_j \pi_j (1\pm \eps') \exp(-\norm{g_1(\va_i) - \vb_i}^2/{{\sigma^*}_1}^2)/{\sigma^*}_1 
% = 1$. 
% The second-to-last equality is a consequence of choosing $\eps$ sufficiently small,
% and $\eps'$ satisfying $1+\eps' < \alpha$. 


% The final equality follows from the facts that (i) the partitions are independent of the noise
% (ii) both Horn's method and the empircal estimate of the standard deviation are consistent, 
% and converge to the true mean.

% It is easy to see that if $\pi^{(r)}_q < (1-3\eps)\pi^{(r)}_{i^*}$, 
% then then all the samples in $H_q$ will be reassigned to $H_{i^*}$.

% \emph{Noiseless setting:}



% \emph{With Noise:}

% Our proof proceeds in $2$ steps:

% First, the initial clustering $\cH := \{ H_1, \dots, H_{M} \}$ is such that each of the $H_i$ is either a subset of $G_j$ for some $j$ or entirely consists of outliers.
% This is because the only $\tau$-connected subsets of the data either consist of samples that are entirely contained in one of the $G_i$ or (possibly) the set of outliers. 
% Second, In each iteration, the mass on the ground truth clusters concentrates. 

% To see this, suppose that during the $r^{th}$ iteration,
% the weights for the $M$ hypotheses are given by $\pi^{(r)}_1, \dots, \pi^{(r)}_{M}$.
% Let $i^* := \argmax_i \pi_i^{(r)}$. 
% Of these, suppose without loss of generality that for some $t \geq 1$, 
% hypotheses $H_1, \dots, H_t \subset G_1$,
% and $\cup_{i=1}^t H_i = G_1$. 
% Then, 
% \begin{enumerate}
%     \item If $\pi^{(r)}_{i^*}$ is sufficiently large (larger than $(1+3\eps)$ times the second largest in the set $\{ \pi_i^{(r)} \}_{i=1}^{M}$), then in the M-step, every sample that is $\tau$-close to  $H_{i^*}$ gets assigned to $i^*$. \label{item:large_sufficient}
%     \item Since each of the ground-truth sets are $\tau$-connected, there are always samples close to the largest cluster which will keep getting accumulated. 
%     \item Since the noise $\eps$ is much smaller than $\tau$, we see that the variance cannot 
% \end{enumerate}
%     To see \Cref{item:large_sufficient}, observe that 
%     This is because for any $(\va_i, \vb_i)$ which is $\tau$-close to $H_{i^*}$, 
%     $\argmax_j W^{(r)}_{i,j;\tau} 
%     = \argmax_j \pi^{(r)}_j \phi^{(r)}_j(\vb_i \mid \va_i) 
%     = \argmax_j \pi^{(r)}_j \exp(\norm{h_j(\va_i) - \vb_i}^2/{\sigma^{(r)}_j}^2)/\sigma^{(r)}_j = \argmax_j \pi^{(r)}_j (1\pm \eps) \exp(\norm{g_1(\va_i) - \vb_i}^2/{{\sigma^*}_1}^2)/{\sigma^*}_1 
%     = i^*$. 
%     The final equality follows from the fact that 
%     each of the $h_j$ are 


% Then, it is easy to see that if some point $(\va_i, \vb_i) \in H_1$, 
% line $18$ of the algorithm will assign the point $p_j$ to the hypothesis indexed by $f(i) := \argmax_j W_{i,j;\tau}^{(r)}$. 
% The convention the algorithm uses is that $f(i)$ will be the smallest index
% among all the possible candidates which achieve the largest value. 
% We will show that if $\pi^{(r)}_1$ is sufficiently large,
% then all the mass gets concentrated in $H_1$.
% If this is not the case, then $\pi^{(r)}_1$ will eventually
% become sufficiently large. 
% To see the first claim, we make the following observations: 
% (i) Since each $H_i$ is sufficiently large, and independent of the noise. The sample variance of each of the sets $H_1, \dots, H_t$, $\sigma^{(r)}_{i} = \sigma_1 (1 \pm \epsilon)$. 
% (ii) If $\pi^{(r)}_1 \geq (1+\eps) \pi^{(r)}_{2}$, then every sample in $H_1 \cup \dots \cup H_t$ goes to $H_1$. 


% $
% = \argmax_j  \frac{ \pi_j^{(r)}\phi_k^{(r)}(\vb_i | \va_i)}{\sum_{j=1}^g \pi_j^{(r)} \phi_j^{(r)}(\vb_i | \va_i) } 
% \cdot \mathbf{1}(d_{\text{cluster}}(H_j, (\va_i, \vb_i)) < \tau)$.
% This is nonzero only if the distance from $H_j$ to  $(\va_i, \vb_i)$ is at most $\tau$.
% This ensures that the point $(\va_i, \vb_i)\in G_1$ 
% cannot be assigned to any $G_j$ where $j \neq 1$. 
% If the value is indeed nonzero, then in the next iteration $r+1$, 
% the point $(\va_i, \vb_i)$ will be assigned to the hypothesis $H_j$
% where $j = \argmax_{j \in [t]} \pi_j^{(r)}\phi(0,{\sigma^{(r)}}_j^2)$.
% We put the hypothesis in the smallest index cluster if all entries are the same.
% However, since with probability 
% \snote{1. show big clusters get bigger. 
% 2. If equal sized cluster then the preference is to a lower index.}

% Since $|H_i| \geq \Omega(\frac{1}{\eps^2} \log(1/\delta))$ we know that Horn's Method recovers a hypothesis $h_i$ that is close to $g_j$ (see \cite{}). 
% \snote{don't talk about $h_i$, these will keep getting updated later. $H_i$ depends on the original noise gaussian}

% \hide{\new{
% We will show that given a good initialization,
% it is possible to recover the right hypotheses.
% To this end, we demonstrate the following.

% \emph{1. The ``good hypotheses" are never eliminated:}
% To see this, observe that the error a point $\vp$ makes with respect to the target hypothesis is small.
% This is because the rotations are well-separated. 
% Additionally, note that the likelihood of such a point is going to be nonzero.


% \emph{2. Any hypothesis that makes an error of more than $10\tau$ with the original hypothesis is eliminated.}
% To see this, suppose to the contrary that there is an h which is far from all the $g_1, .., g_|G|$.but makes an error of $\leq \tau$ for each of these.This means there is at least one $G_i$ which overlaps with $h$ significantly.
% But this means $h(x) - y = g(x) - y \pm \tau$ and so $h(x) - g(x) = O(\tau)$.
% but this in turn means that $h$ and $g$ are close.so the number of points that $h$ explains has to be smaller than \new{???}.If so, it gets eliminated..

% \emph{3. Among the good hypotheses the points that correspond to that object eventually collect}
% Let the ground truth be let $p \in G_i$ and suppose the samples are


% \snote{Need to first find weights, then cluster together etc. This will help collect things. Which will eventually converge. }

% }
% We will discuss this in the noiseless setting first.

% \paragraph{Noiseless}

% We know from the setting of the problem (\Cref{set:problem})
% that $|G_i| \geq \gamma |S|$. 

% Let $\cH_{\geq}$ denote the subset of $\cH$ such that for every $h \in \cH_{\geq}$,
% $|H_0(h)| \geq \gamma |S|$, where 
% $H_\eta(h) := \{ (x, y) \in S \mid \err(h; \{(x, y)\}) \leq \eta \}$. 
% Now, since $S$ is partitioned into $G_1, \dots, G_k$, 
% it must be the case that each $H_0(h)$ has some overlap with some of the $G_i$. 
% Since the setting is non-degenerate (\Cref{item:NdO} from \Cref{set:problem}), 
% If $|H_0(h) \cap G_i| \geq (d+1)$ where $d$ is the dimension (in our case a constant),
% then $h \equiv g_i$. 
% Otherwise $|H_0(h)| \leq (d+1) k$. 
% However, since $m > (d+1) k/\gamma$, and $|H_0(h)| \geq \gamma |S|$,
% we see that $h \notin \cH'$.
% Hence every $h \in \cH'$ is a ground truth hypothesis.
% Also, no ground truth hypothesis is removed, since $G_i \subset H_0(g_i)$ for every $i \in [k]$. \snote{$\cH'$ and $\cH_{\geq}$. Make them the same.}

% \paragraph{Randomly Selected Arbitrary Outliers}

% Suppose an $\eps$ fraction of the samples $S$ are corrupted arbitrarily,
% but the location of these corruptions is uniform at random
% (this ensures that no object gets completely hidden).

% In the absence of any other noise, the previous argument still goes through.
% \snote{Okay, but how will you ensure good initial estimates via clustering?
% I think the right clustering strategy will not cluster the outliers with the inliers
% unless they are close to being inliers, in which case it does not matter.}
% Let $I$ denote the set of inliers, and $O$ the set of outliers, and $I \cup O = S$.
% If a hypothesis $h$ satisfies 
% $|H_0(h) \cap H_0(g)| \geq \Omega((d+1)/(1-\eps) \log(1/\delta))$ for some $g \in \cG$, 
% then, with probability $1-\delta$, $|H_0(h) \cap H_0(g) \cap I| \geq \Omega(d+1)$. 
% in which case, $h \equiv g$. 
% If there is no $g$ for which $|H_0(h) \cap H_0(g)| \geq \Omega((d+1)/(1-\eps) \log(1/\delta))$,
% then it must be that $|H_0(h)| \leq O((k (d+1) / (1-\eps)) \log(1/\delta))$.
% As long as $|S|$ is large enough, once again, 
% we have a contradiction and $h$ should have been removed.
% \snote{also consider adversarial noise}

% \new{\paragraph{Bounded Additive Noise}

% Suppose each $g_i$ satisfies $\err(g_i; G_i) \leq \eta$. 
% We know from the setting of the problem (\Cref{set:problem}) 
% that $|G_i| \geq \gamma |S|$. 
% Let $\cH_{\geq}$ denote the subset of $\cH$ such that for every $h \in \cH_{\geq}$,
% $|H_\eta(h)| \geq \gamma |S|$.

% Now, since $S$ is partitioned into $G_1, \dots, G_k$, 
% it must be the case that each $H_\eta(h)$ has some overlap with some of the $G_i$. 

% Since the setting is non-degenerate (\Cref{item:NdO} from \Cref{set:problem}), 
% \new{If $|H_\eta(h) \cap G_i| \geq \gamma' |S|$ then $\err(h, G_i) \leq (\gamma/\gamma')$.} 
% Otherwise $|H_\eta(h)| \leq \gamma' k |S|$. 
% However, since $m > |S|/k\gamma'$, and $|H_\eta(h)| \geq \gamma |S|$,
% we see that $h \notin \cH'$.
% Hence every $h \in \cH'$ is a ground truth hypothesis.

% Also, no ground truth hypothesis is removed, 
% since $G_i \subset H_\eta(g_i)$ for every $i \in [k]$. 
% Suppose each for every $g \in \cG$ we have $|H_\eta(h) \cap H_\eta(g)| \leq \alpha |S|$
% and so $|H_\eta(h)| \leq k \alpha |S|$. }
% }

% \end{proof}
